Constant RMR Recoverable Mutex under System-wide Crashes

We design two Recoverable Mutual Exclusion (RME) locks for the system-wide crash model. Our first algorithm requires only $O(1)$ space per process, and achieves $O(1)$ worst-case RMR complexity in the CC model. Our second algorithm enhances the first algorithm to achieve (the same) $O(1)$ space per process and $O(1)$ worst-case RMR complexity in both the CC and DSM models. Furthermore, both algorithms allow dynamically created threads of arbitrary names to join the protocol and access the locks. To our knowledge, these are the only RME locks to achieve worst-case $O(1)$ RMR complexity assuming nothing more than standard hardware support. In light of Chan and Woelfel's $\Omega(\log n / \log\log n)$ worst-case RMR lower bound for RME in the individual crash model, our results show a separation between the system-wide crash and individual crash models in worst-case RMR complexity in both the CC and DSM models.

==> cc_alg_old.tex <==
\section{The RME Algorithm for CC} 
\label{sec:mainalg}

Our algorithm, which implements a recoverable mutual exclusion lock $\L$, 
for the CC model under the system-wide crash failure model, is specified in Figure~\ref{algo:fullcrash}.
To  present the intuition behind how the algorithm works,
we first describe in Section~\ref{sec:highlevel} the crucial high level ideas underlying the algorithm,
including the purpose of the variables employed in the algorithm.
Then, in Section~\ref{sec:commentary}, we present the line-by-line commentary.
In the next section, we present an invariant-based proof of correctness of our algorithm.

\subsection{High level ideas} \label{sec:highlevel}

The algorithm uses the following persistent (NVM) variables.
Some are shared and the others, subscripted with $p$, are local to process $p$.

\begin{itemize}
	\item
	\underline{$\seq$ and $\sp$}: $\seq$ stores an unbounded sequence number that grows monotonically,
	and the local variable $\sp$ holds what process $p$ believes to be the current sequence number.
	If $p$ crashes and subsequently restarts, it increases $\seq$ to $\sp +1$.
	
	\item
	\underline{$\lck[0]$, $\lck[1]$, $\lck[2]$}: 
	These are three instances of the base lock that we discussed in the previous section and presented in Figure~\ref{algo:qlock}.
	Each process incurs $O(1)$ RMR complexity on CC machines when using the lock.
	To compete with other processes in order to obtain the ownership of the CS, $p$ uses the lock numbered $\sp \% 3$.
	
	\item
	\underline{$\stopwait[0]$, $\stopwait[1]$, $\stopwait[2]$}:
	These are boolean variables and the variable $\stopwait[\sp \% 3]$ denotes whether $\lck[\sp \% 3]$ is in good condition or not.
	That is to say that, if a crash occurred while a process was actively using the lock $\lck[\sp \% 3]$ and the lock was not subsequently reset, 
	then the lock is not in good condition and hence should not be used to gain access to the CS.
	
	\item
	\underline{$\cso$}: 
	This variable stores the name of the process in the CS of the implemented recoverable lock $\L$ (i.e., the real CS and not that of any of the three base lock).
	Its value is $\bot$ if no process is in the CS of $\L$.
	
	\item
	\underline{$\inuse_p$}: This boolean local variable holds {\em true} while $p$ executes the algorithm.
	Therefore, if $p$ jumps to the Remainder section because it crashed while executing the algorithm,
	$\inuse_p$ has $\true$.
	On the other hand, if $p$ completes the algorithm normally (e.g., without crashing),
	$\inuse_p$ has $\false$ when $p$ reaches the Remainder section.
	
% TODO: Need to be sure about below lines because we might need these in the description of base lock instead.
%	\item
%	\underline{$\nodes_p$}: This local variable contains a pointer to a node, 
%	where a node has a single boolean field.
%	When $p$ competes for one of $\lck[0]$, $\lck[1]$, or $\lck[2]$, 
%	it writes {\em false} in its node and enqueues it in the lock's wait-queue.
%	When $p$ releases a lock, it writes {\em true} in the node to signal to the process $q$ behind $p$ in the wait-queue
%	that $q$ now owns the lock. See Figure~\ref{algo:baselock} and its explanation in Section~\ref{sec:baseintuit} for details.
%	
%	
%	\item
%	\underline{$\prevnode_p$}: When $p$ enqueues its node in the wait-queue of a base lock,
%	it remembers the pointer to the node immediately ahead of it in the wait-queue by storing
%	that pointer in $\prevnode_p$. See Figure~\ref{algo:baselock} and its explanation in Section~\ref{sec:baseintuit} for details.
\end{itemize}

The idea is that, in order to compete for the recoverable lock $\L$,
each process $p$ reads into $\sp$ the sequence in $\seq$ and attempts to acquire 
the base lock $\lck[\sp \% 3]$ (by executing $\lck[\sp \% 3].\tryprocp()$).
For example, if processes $p$ and $q$ compete for $\L$ when the sequence number is 10,
they try to acquire $\lck[10 \% 3]$ (or $\lck[1]$).
If there are no crashes, then each process acquires $\lck[1]$, enters the CS of $\L$,
and then releases $\lck[1]$.
Thus, $p$ and $q$ enter the CS of $\L$ one after the other and return to the Remainder section.

For a more complex scenario, suppose that the system crashes while $p$ and $q$ are competing for $\lck[1]$.
The crash wipes out these process' CPU registers, thereby rendering $\lck[1]$ unusable in the future.
When one of these processes, say $p$, subsequently restarts and enters $\recoverprocp()$ of $\L$,
it infers from the value of $\true$ in $\inuse_p$ that it must have crashed while executing the algorithm.
So, $p$ advances $\seq$ by writing 11 and goes on to acquire $\lck[11 \% 3]$, or $\lck[2]$, if necessary.
However, suppose that a third process $r$ executes the algorithm before $p$ changes $\seq$ to 11.
Since $r$ has no previous context, when it reads 10 in $\seq$, it simply writes 10 in $\myseq_r$
and competes for $\lck[10 \% 3]$ (i.e., in $\lck[1]$), which could be stuck, but then $r$ doesn't know that.
If $p$ now takes steps, it writes 11 in $\seq$ and proceeds to compete for $\lck[11 \% 3]$ (i.e., $\lck[2]$).
Thus, at this point, there are processes waiting at two different locks, namely, $\lck[1]$ and $\lck[2]$.
To prevent $r$ from being stuck forever at $\lck[10 \% 3]$, 
we require that while waiting in the $\tryproc{r}()$ procedure of $\lck[10 \% 3]$, $r$ parallely also checks whether $\stopwait[10 \% 3]$ changes to $\true$.
On noticing a change in $\stopwait[10 \% 3]$, $r$ can promptly switch to $\lck[11 \% 3]$.

Could there be a scenario where processes could be waiting at three locks?
The answer is no.
To see this, suppose that a system-wide crash occurs when $\seq$ has some value $v$.
Processes that have not witnessed the value $v$ in $\seq$ in the past (such as process $r$ in the previous scenario)
as well as processes that saw $v$ in $\seq$ but exited the algorithm normally
will proceed to $\lck[v \% 3]$, while those that had seen $v$ in $\seq$ and experienced the crash
write $v+1$ in $\seq$ and wait at  $\lck[(v+1) \% 3]$.
Thus, there is no possibility of any process flocking to a third lock.
In particular, of the three base locks employed in the algorithm, we can be certain that
no process waits at $\lck[(v-1) \% 3]$.
Since this lock could be stuck from prior crashes, now is the ripe time to reset and keep it ready for future use;
so, $p$ resets $\lck[(v-1) \% 3]$ as it changes $\seq$ from $v$ to $v+1$.
This observation that three base locks suffice
and that $\lck[(v-1) \% 3]$ should be reset when changing $\seq$ from $v$ to $v+1$
is a crucial insight in our algorithm.
%There are other important ideas, but we will explain these as we do the line-by-line commentary.

%\section{The Algorithm} \label{sec:algo}
%We present our abortable RME algorithm in Figure~\ref{algo:reccc2lock}. 
%The algorithm is designed for an unknown and arbitrary number of processes.
%All the shared variables used by our algorithm are stored in the NVM.
%Variables with a subscript of $p$ to their name are variables local to the process $p$.
%When the name of such variables is in all small letters, they are stored in $p$'s registers, otherwise, they are stored in the NVM.
%We assume that the CS is an idempotent block of code, which allows a process to re-execute it from start even if the process crashes in the middle of the CS.

\setcounter{linecounter}{0}
\begin{figure}[!ht]
	\begin{footnotesize}
		\hrule
		\vspace{-3mm}
		\begin{tabbing}
			\hspace{0in} \=  \hspace{0.2in} \= \hspace{0.1in} \=  \hspace{0.2in} \= \hspace{0.2in} \= \hspace{0.2in} \=\\
			{\bf Shared variables (stored in NVM)} \\ 
			\hspace{0in} \=  \hspace{0.1in} \= $\seq \in \mathbb{N}$, initially $1$. \\
			\> \> $\mlock[0 \cdots 2]$ is an array of base mutual exclusion locks, as implemented in Figure~\ref{algo:qlock}. \\
			\> \> $\stopwait[0 \cdots 2]$ is an array of booleans, each initially {\em false}. \\
			\> \> $\barrier$ stores a process identifier or $\none$, initially $\none$.  \\
			\> {\bf Persistent variables local to process $p$ (stored in NVM)} \\
			\> \> $\inusep$ is a boolean, initially {\em false}. \\
			\> \> $\myseqp \in \mathbb{N}$, initially $1$. 
		\end{tabbing}
		
		\begin{minipage}[t]{.95\linewidth}%{.5\linewidth}
			\begin{tabbing}
				\hspace{0in} \= \hspace{0.25in} \= \hspace{0.2in} \=  \hspace{0.2in} \= \hspace{0.2in} \=\\
				\> \procline{fullcrash:rem:1} \> {\texttt{Remainder Section}} \\
				\\
				\> \> \underline{\texttt{procedure $\tryprocp()$}}\\
				\> \procline{fullcrash:try:1}\> $\inusep \gets \true$ \\
				\> \procline{fullcrash:try:2} \> $\myseqp \gets \seq$ \\
				\> \procline{fullcrash:try:3} \> $\mlock[\myseqp \% 3].\tryprocp()$ \hspace{.2in} $\parallel$ \hspace{0.1in} \waittill $\stopwait[\myseqp \% 3] = \true$  \\
				\> \procline{fullcrash:try:4} \> \ifcode $\seq \neq \myseqp$: \goto Line~\refln{fullcrash:try:8} \\
				\> \procline{fullcrash:try:5} \> \waittill $\csowner \isequal \perp$ \hspace{.1in} $\parallel$ \hspace{.1in} \waittill $\stopwait[\myseqp \% 3] = \true$ \\
				\> \hspace{1.55in} \goto Line~\refln{fullcrash:try:8} \\
				\> \procline{fullcrash:try:6} \> \ifcode $\cas(\csowner, \perp, p)$: \return \gotocs \\
				\> \procline{fullcrash:try:7} \> \ifcode $\seq \neq \myseqp$: \\
				\> \procline{fullcrash:try:8} \> \> $\myseqp \gets \myseqp + 1$ \\
				\> \procline{fullcrash:try:9} \> \> $\mlock[\myseqp \% 3].\tryprocp()$ \\
				\> \procline{fullcrash:try:10} \> \> \waittill $\csowner \isequal \perp$ \\
				\> \procline{fullcrash:try:11} \> \> \ifcode $\cas(\csowner, \perp, p)$: \return \gotocs \\
				\> \procline{fullcrash:try:12} \> \waittill $\csowner \isequal \perp$ \\
				\> \procline{fullcrash:try:13} \> $\csowner \gets p$ \\
				\> \procline{fullcrash:try:14} \> \return \gotocs \\
				\\
				\> \procline{fullcrash:cs:1} \> {\texttt{Critical Section}} \\
				\\
				\> \> \underline{\texttt{procedure $\exitprocp()$}}\\
				\> \procline{fullcrash:exit:1} \> \ifcode $\myseqp \isequal \seq$: \\
				\> \procline{fullcrash:exit:2} \> \> $\mlock[\myseqp \% 3].\exitprocp()$ \\
				\> \procline{fullcrash:exit:3} \> $\csowner \gets \none$ \\
				\> \procline{fullcrash:exit:4} \> $\inusep \gets \mbox{\it false}$ \\
				\\
				\> \> \underline{\texttt{procedure $\recoverprocp()$}}\\
				\> \procline{fullcrash:rec:1} \> \ifcode $\inusep \wedge \seq \isequal \myseqp$: \\
				\> \procline{fullcrash:rec:2} \> \> $\mlock[(\myseqp - 1) \% 3].\initializep()$ \\ 
				\> \procline{fullcrash:rec:3} \> \> $\stopwait[(\myseqp - 1) \% 3] \gets \mbox{\it false}$ \\
				\> \procline{fullcrash:rec:4} \> \> $\seq \gets \myseqp + 1$ \\
				\> \procline{fullcrash:rec:5} \> \> $\stopwait[\myseqp \% 3] \gets \true$ \\
				\> \procline{fullcrash:rec:6} \> \ifcode $\csowner \isequal p$: \return \gotocs \\
				\> \procline{fullcrash:rec:7} \> $\inusep \gets \mbox{\it false}$ \\
				\> \procline{fullcrash:rec:8} \> \return \gotorem
			\end{tabbing}  
		\end{minipage}
		\vspace*{-2mm}
		\captionsetup{labelfont=bf}
		\caption{Algorithm for an RME lock $\L$ for an arbitrary number of processes of arbitrary names, for CC machines. Code shown for a process $p$.} 
		\label{algo:fullcrash}
		\hrule
	\end{footnotesize}
\end{figure}

\subsection{Line-by-line commentary} \label{sec:commentary}
In this section we informally describe the working of our algorithm presented in Figure~\ref{algo:fullcrash}.
We first describe how a process $p$ would execute the algorithm in the absence of a crash, 
and then proceed to explain the working of the algorithm in presence of a crash.

\subsubsection*{Crash-free attempt.}
A process $p$ starts an attempt to enter the CS from the Remainder Section by invoking the $\tryprocp()$ procedure.
At Line~\refln{fullcrash:try:1}, $p$ sets $\inusep$ to $\true$ making a note to itself that it has started an attempt.
Subsequently, $p$ reads the current sequence number $\seq$ into its local variable $\myseqp$ at Line~\refln{fullcrash:try:2}, and proceeds by trying to acquire the corresponding lock $\mlock[\myseqp \% 3]$ at Line~\refln{fullcrash:try:3}.
While executing $\lck[\myseq_p \% 3].\tryprocp()$, 
$p$ simultaneously monitors the value of the corresponding stop flag, $\stopwait[\myseqp\% 3]$, by interleaving its steps between the try method and the \waittill at Line~\refln{fullcrash:try:3}.
If $\myseqp\%3$ is indeed the current lock, then $p$'s try attempt will eventually succeed.
Otherwise, if another process $q$ that previously crashed while active in the lock with sequence number $\myseqp$ restarts, it will increment $\seq$ and set the flag  $\stopwait[\myseqp\% 3]$ to {\em true}.
When $p$ finishes Line 4, it could have been because it successfully obtained the lock or because the stop flag was raised.
Thus, it checks whether the sequence number $\seq$ was incremented at Line 5, if so it abandons the $\lck[\myseqp\%3]$ and proceeds to update its sequence number at Line 9 and proceeds to try to obtain the newly installed lock (as we explain later).
Otherwise, if $\myseqp$ is still current (i.e. it still equals $\seq$), then $p$ waits for the CS to become freed by spinning on $\csowner$ at Line 6.
Once again, $p$ is aware that the sequence number could be updated, so it simultaneously monitors $\stopwait[\myseqp\%3]$ and (just as before) proceeds to Line 9 if the stop flag gets raised.
If $p$ eventually finds the CS vacated (i.e. $\csowner = \perp$ at Line~\refln{fullcrash:try:5}), it tries to establish ownership of the CS by CASing its name into the $\csowner$ field at Line~\refln{fullcrash:try:6}.
If $p$ succeeds in the \cas, then it moves to the CS.
Otherwise, as we explain in the following, there could be two reasons that $p$ failed in the \cas\ after having read that the CS is empty at Line~\refln{fullcrash:try:5}.
In the first case, the lock used by $p$ must have been an older lock that was part of a crash before $p$ enqueued itself into it,
and subsequently a new lock was installed that allowed another process to enter the CS (all of this not noticed by $p$).
In the second case $p$ itself was enqueued in the latest lock, however, it lost to another process $q$ that had enqueued itself into a older lock (just like $p$ in the first case above).
To find out which of the above two cases caused this \cas\ failure, $p$ compares $\seq$ with $\myseqp$ at Line~\refln{fullcrash:try:7}.
If the two are the same, $p$ knows it is in the right lock, hence, it goes to Line~\refln{fullcrash:try:12} to wait for its turn to occupy the CS.
Otherwise, $p$ tries for the latest active base lock next, hence, it goes to Line~\refln{fullcrash:try:8}.

From the above description, we see that $p$ could reach Line~\refln{fullcrash:try:8} in three different ways: from Line~5, Line~6, or Line~8. 
In all the cases, $p$ knows that the sequence number increased after its execution of Line 3.
Since, $p$ knows that the sequence number could go up only once between two crashes (an invariant maintained by our algorithm), it increments $\myseqp$ by 1 (Line~\refln{fullcrash:try:8}) to the current value of $\seq$.
This time, when $p$ tries for the lock $\lck[\myseqp\%3]$ at Line~10, it is guaranteed to eventually succeed (if there is no system-wide crash), and thus does not need to simultaneously monitor a stop flag.
At Line~\refln{fullcrash:try:10} $p$ waits to ensure that the CS is empty.
It needs to ensure this for one of two reasons: either a process acquired the CS before the crash and still continues to do so,
or a process succeeded in the \cas\ at Line~\refln{fullcrash:try:6} by coming through a lock before it was replaced by the current lock that $p$ came from.
Once $p$ is past Line~\refln{fullcrash:try:10}, it attempts to \cas\ its own name into $\csowner$ if the CS is still empty.
If $p$ succeeds in the \cas, then it moves to the CS.
Otherwise $p$ failed only because some other process must have succeeded in the \cas\ at Line~\refln{fullcrash:try:6} as described above.
$p$ waits one more time at Line~\refln{fullcrash:try:12} to ensure that the CS is empty.
Once $p$ reaches Line~\refln{fullcrash:try:13} it is sure that it reached the line by enqueuing into the latest active lock and there could not be any more competition to it.
Hence it writes its own name into $\csowner$ and moves to CS (Line~\refln{fullcrash:try:14}).

In the $\exitprocp()$ procedure, $p$ first checks if the base lock that it queued up and entered the CS from is still the active lock (Line~\refln{fullcrash:exit:1}).
If it is indeed still the active lock, $p$ executes the $\exitprocp()$ procedure of that lock at Line~\refln{fullcrash:exit:2}.
Otherwise, $p$ knows that it is no longer in the queue of the lock it used and hence doesn't execute the $\exitprocp()$ method of that lock.
At Line~\refln{fullcrash:exit:3} $p$ informs other processes that it is giving up the CS by writing $\perp$ to $\csowner$.
Finally, at Line~\refln{fullcrash:exit:4} $p$ sets $\inusep$ to $\false$ to complete its attempt.

\subsubsection*{Recovery from a crash.}
We now discuss what happens when $p$ crashes while executing an attempt.
The idea behind our algorithm is to keep an active instance of the base lock and the number in $\seq$ determines which of the three instances is active.
Therefore, in any configuration, $\mlock[\seq \% 3]$ is the active base lock.
This idea guides a process on whether after a crash it needs to setup a new lock or not.
Thus, at Line~\refln{fullcrash:rec:1}, $p$ determines if it took any meaningful steps prior to the crash, and if so, whether it might have attempted to queue up in the currently active base lock.
If $\inusep = \false$, $p$ is sure that it didn't take any meaningful steps before the crash and hence continues to Line~\refln{fullcrash:rec:6} of the procedure
(from there it is sure to find $\csowner \neq p$ and thus will return to the Remainder completing the attempt).
If $\inusep = \true$ but $\myseqp \neq \seq$, then $p$ knows that it no longer needs to setup a new lock because either a new lock was already setup
or the currently active lock is not the one that $p$ queued itself into.
Thus, $p$ would continue to Line~\refln{fullcrash:rec:6}.
In the case where $\inusep = \true$ and $\myseqp = \seq$, $p$ might have enqueued itself into $\mlock[\seq \% 3]$ at either of Lines~\refln{fullcrash:try:3} or \refln{fullcrash:try:9}.
Hence, assuming that $p$ itself has broken the queue structure of $\mlock[\seq \% 3]$, it moves to setup a new lock at Lines~\refln{fullcrash:rec:2}\upto\refln{fullcrash:rec:5}.
Our algorithm maintains the invariant that $\mlock[(\seq + 1) \% 3]$ is always initialized, i.e., the next instance of $\mlock$ is always kept ready to use.
Therefore, before installing the next lock in sequence, $p$ readies the lock after the next lock in sequence to maintain the invariant.
To this purpose, at Line~\refln{fullcrash:rec:2}, $p$ first resets the lock $\mlock[(\myseqp - 1) \% 3]$, 
which is the lock coming up after the next lock in sequence (i.e., lock numbered $(\seq + 2) \% 3$ or $(\seq - 1) \% 3$ is the lock coming up after the next lock in sequence).
$p$ then resets the $\stopwait$ flag associated with lock $\mlock[(\myseqp - 1) \% 3]$ at Line~\refln{fullcrash:rec:3}.
Next $p$ moves to signal that $\lck[\myseqp \% 3]$ should no longer be used, therefore, it increments $\seq$ by $1$ at Line~\refln{fullcrash:rec:4}.
It then sets $\stopwait[\myseqp \% 3]$ to $\true$ (at Line~\refln{fullcrash:rec:5}) so that any processes that queued up at lock $\lck[\myseqp \% 3]$ in the time between the previous crash and now know that they should move to the next lock in sequence, i.e., $\lck[\seq \% 3]$.
An invariant our algorithm maintains is that between two consecutive crashes, the value of $\seq$ is incremented at most once.
To see how that is achieved consider the following example. 
Suppose $p$, $q$, and $r$ committed to the value 10 by reading $\seq$ at Line~\refln{fullcrash:try:2} and noting into their respective variables $\myseqp$, $\myseq_q$, and $\myseq_r$.
Assume that a crash occurs after that and $p$ and $q$ restart immediately actively taking steps.
$p$ and $q$ both read $\seq = \myseq_p$ and $\seq = \myseq_q$ and thus execute Lines~\refln{fullcrash:rec:2}-\refln{fullcrash:rec:3} one after another.
After that $q$ executes Line~\refln{fullcrash:rec:4} first to set $\seq$ to 11 for the first time.
Following this, $p$ will execute Line~\refln{fullcrash:rec:4} at most once before the next crash, 
and that step wouldn't change the value of $\seq$ because $p$ would attempt to set it to 11, a value $\seq$ already holds. 
Also, following the step by $q$, no matter when $r$ starts taking steps, it will always find $\seq = 11$ which is not the same as what $\myseq_r$ held prior to the crash.
Hence, $r$ would never change the value of $\seq$.
Thus, with the execution of Line~\refln{fullcrash:rec:5}, $p$ completes the repair and moves to execute Line~\refln{fullcrash:rec:6}.

At Line~\refln{fullcrash:rec:6} $p$ checks if it acquired access to the CS prior to the crash by checking if $\csowner = p$.
If so, $p$ moves to the CS  by returning $\gotocs$ from $\recoverprocp()$.
Otherwise, $p$ is sure that it has repaired any issues that might have caused due to the crash and it can't go in the CS any more in the current attempt.
Thus it sets the $\inusep$ flag to $\false$ (Line~\refln{fullcrash:rec:7}) to signal the end of the attempt and returns $\gotorem$ (Line~\refln{fullcrash:rec:8}) to go back to the Remainder.

In the above, Line~\refln{fullcrash:rec:6} may put $p$ into the CS, hence satisfying the CSR property.
Thus, in the $\exitprocp()$ procedure $p$ checks if it entered the CS normally or due to the CSR property as mentioned above.
If $p$ finds that $\seq = \myseq_p$ at Line~\refln{fullcrash:exit:1}, it infers that it entered the CS normally, 
and hence executes the $\exitprocp()$ procedure of $\mlock[\myseq_p \% 3]$ at Line~\refln{fullcrash:exit:2}.
Otherwise, $p$ knows that it is no longer in the queue of the lock it used and hence doesn't execute $\exitprocp()$.
At Line~\refln{fullcrash:exit:3} $p$ informs other processes that it is giving up the CS by writing $\perp$ to $\csowner$.
Finally, at Line~\refln{fullcrash:exit:4} $p$ sets $\inuse_p$ to $\false$ to complete its attempt.

\subsubsection*{Execution of $\recoverprocp()$ when $\status_p = \good$.}
Our algorithm maintains an invariant that if $p$ is not active in an attempt during a configuration,
then $\activep = \false$ and $\csowner \neq p$.
Thus, if $p$ invokes a call to $\recoverprocp()$ from the Remainder section when $\status_p = \good$, 
the \ifcode conditions at Lines~\refln{fullcrash:rec:1} and \refln{fullcrash:rec:6} are not met.
Therefore, $p$ executes Line~\refln{fullcrash:rec:7} which sets $\inusep$ to $\false$ and returns $p$ back to the Remainder (Line~\refln{fullcrash:rec:8}).


==> dsm_alg_old.tex <==
\section{The RME algorithm for DSM}\label{sec:dsmalg}

The RMR complexity of the RME algorithm presented in the last section is $O(1)$ in CC machines, but unbounded in DSM machines.
In this section we present an algorithm that has $O(1)$ RMR complexity in both DSM and CC machines.
We have been able to design this DSM/CC algorithm (DSM algorithm, for short) to be so similar to the CC algorithm that the correctness of the DSM algorithm follows from that of the CC algorithm.
Below, we first describe the ideas behind how we transformed the CC algorithm into an efficient DSM algorithm, and then present the technical details.


\setcounter{linecounter}{0}
\begin{figure}[!ht]
	\begin{footnotesize}
		\hrule
		\vspace{-3mm}
		\begin{tabbing}
			\hspace{0in} \=  \hspace{0.2in} \= \hspace{0.1in} \=  \hspace{0.2in} \= \hspace{0.2in} \= \hspace{0.2in} \=\\
			{\bf Shared variables (stored in NVM)} \\ 
			\hspace{0in} \=  \hspace{0.1in} \= $\seq \in \mathbb{N}$, initially $1$. \\
			\> \> $\alock[0 \cdots 2]$ is an array of base mutual exclusion locks, as implemented in Figure~\ref{algo:dsmqlock}.  \\
			\> \> $\stopwait[0 \cdots 2]$ is an array of boolean signal objects, as implemented in Figure~\ref{algo:dsmsignal}, each initially {\em false}. \\
			\> \> $\barrier$ is a capturable object, as implemented in Figure~\ref{algo:capturable}, initially $\none$. \\
			\\
			\> {\bf Persistent variables local to process $p$ (stored in NVM)} \\
			\> \> $\inusep$ is a boolean, initially {\em false}. \\
			\> \> $\myseqp \in \mathbb{N}$, initially $1$. 
		\end{tabbing}
		
		\begin{minipage}[t]{.95\linewidth}%{.5\linewidth}
			\begin{tabbing}
				\hspace{0in} \= \hspace{0.25in} \= \hspace{0.2in} \=  \hspace{0.2in} \= \hspace{0.2in} \=\\
				\> \procline{dsmfullcrash:rem:1} \> {\texttt{Remainder Section}} \\
				\\
				\> \> \underline{\texttt{procedure $\tryprocp()$}}\\
				\> \procline{dsmfullcrash:try:1}\> $\inusep \gets \true$ \\
				\> \procline{dsmfullcrash:try:2} \> $\myseqp \gets \seq$ \\
				\> \procline{dsmfullcrash:try:3} \> $\alock[\myseqp \% 3].\tryprocp()$ \hspace{.1in}  \\
				\> \procline{dsmfullcrash:try:4} \> \ifcode $\seq \neq \myseqp$: \thencode \goto Line~\refln{dsmfullcrash:try:8} \\
				\> \procline{dsmfullcrash:try:5} \> $\csowner.\mwait{}$ \hspace{.1in} $\parallel$ \hspace{.1in} $\stopwait[\myseqp \% 3].\mwait{}$ \\
				\> \hphantom{{\bf 6.}} \> \hphantom{$\csowner.\mwait{}$ \hspace{.1in} $\parallel$ \hspace{.1in}} \goto Line~\refln{dsmfullcrash:try:8} \\
				\> \procline{dsmfullcrash:try:6} \> \ifcode $\csowner.\mcapture{}$ \thencode \return \gotocs \\
				\> \procline{dsmfullcrash:try:7} \> \ifcode $\seq \neq \myseqp$ \thencode \\
				\> \procline{dsmfullcrash:try:8} \> \> $\myseqp \gets \myseqp + 1$ \\
				\> \refln{dsmfullcrash:try:8}{\bf .1.} \> \> $\alock[(\myseqp - 1) \% 3].\mabandon{}$ \\
				\> \procline{dsmfullcrash:try:9} \> \> $\alock[\myseqp \% 3].\tryprocp()$ \\
				\> \procline{dsmfullcrash:try:10} \> \> $\csowner.\mwait{}$ \\
				\> \procline{dsmfullcrash:try:11} \> \> \ifcode $\csowner.\mcapture{}$ \thencode \return \gotocs \\
				\> \procline{dsmfullcrash:try:12} \> $\csowner.\mwait{}$ \\
				\> \procline{dsmfullcrash:try:13} \> $\csowner.\mwrite{}$ \\
				\> \procline{dsmfullcrash:try:14} \> \return \gotocs \\
				\\
				\> \procline{dsmfullcrash:cs:1} \> {\texttt{Critical Section}} \\
				\\
				\> \> \underline{\texttt{procedure $\exitprocp()$}}\\
				\> \procline{dsmfullcrash:exit:1} \> $x_p \gets \seq$ \\
				\> \procline{dsmfullcrash:exit:2} \> \ifcode $\myseqp \isequal x_p$ \thencode $\alock[\myseqp \% 3].\exitprocp()$ \\
				\> \refln{dsmfullcrash:exit:2}{\bf .1.} \> \ifcode $\myseqp \isequal x_p - 1$ \thencode $\alock[\myseqp \% 3].\mabandon{}$\\
				\> \procline{dsmfullcrash:exit:3} \> $\csowner.\mrelease{}$ \\
				\> \procline{dsmfullcrash:exit:4} \> $\inusep \gets \mbox{\it false}$ \\
				\\
				\> \> \underline{\texttt{procedure $\recoverprocp()$}}\\
				\> \procline{dsmfullcrash:rec:1} \> \ifcode $\inusep \wedge \seq \isequal \myseqp$: \\
				\> \procline{dsmfullcrash:rec:2} \> \> $\alock[(\myseqp - 1) \% 3].\initializep()$ \\ 
				\> \procline{dsmfullcrash:rec:3} \> \> $\stopwait[(\myseqp - 1) \% 3].\mreset{}$ \\
				\> \procline{dsmfullcrash:rec:4} \> \> $\seq \gets \myseqp + 1$ \\
				\> \procline{dsmfullcrash:rec:5} \> \> $\stopwait[\myseqp \% 3].\mset{}$ \\
				\> \refln{dsmfullcrash:rec:5}{\bf .1.} \> \ifcode $\myseqp = \seq - 1$: \thencode $\alock[\myseqp \% 3].\mabandon{}$ \\
				\> \procline{dsmfullcrash:rec:6} \> \ifcode $\csowner.\mread{} \isequal p$ \thencode \return \gotocs \\
				\> \procline{dsmfullcrash:rec:7} \> $\inusep \gets \mbox{\it false}$ \\
				\> \procline{dsmfullcrash:rec:8} \> \return \gotorem
			\end{tabbing}  
		\end{minipage}

		\captionsetup{labelfont=bf}
		\caption{
		Algorithm for an RME lock $\L$ for an arbitrary number of processes of arbitrary names, for DSM machines. Code shown for a process $p$.} 
		\label{algo:dsmfullcrash}
		\hrule
	\end{footnotesize}
\end{figure}


\subsection{The main ideas underlying the DSM algorithm}\label{DSM-overview}

To achieve $O(1)$ RMR complexity for our RME algorithm in the DSM model, we need base mutex locks---$\mlock[i]$ for $i \in [0,2]$---that have $O(1)$ RMR complexity on DSM machines.
We obtain these using the algorithm from Figure~\ref{algo:dsmqlock}.
Beyond this simple change, there are several places in our recoverable algorithm of Figure~\ref{algo:fullcrash} where a process busy-waits and incurs unbounded RMRs on a DSM machine.
We devise three ideas that transform each such busy-wait into a method that incurs only $O(1)$ RMRs on a DSM machine.
We describe these ideas below.


\begin{enumerate}
\item
The busy-waiting on $\csowner$ at Lines 6, 11, and 13 of the earlier algorithm incurs unbounded RMRs on a DSM machine since the variable $\csowner$ must reside in a memory partition that is remote to all but one process.
To overcome this difficulty, we have introduced a new object, which we call a {\em capturable object}, that supports a method for each operation the algorithm performs on $\csowner$, and implemented the object so that each of these methods incurs only $O(1)$ RMRs. More specifically, the shared variable $\csowner$ of the CC algorithm is replaced by a capturable object $\csownerdsm$ in our DSM algorithm and the steps ``\waittill $\csowner \isequal \perp$'' (at Lines 6, 11, and 13), ``$\csowner \gets \none$'' (at Line 19), ``read $\csowner$'' (at Line 26), ``$\csowner \gets p$'' (at Line 14), and ``CAS$(\csowner, \bot, p)$'' (at Lines 7 and 12) of the earlier algorithm are replaced, respectively, by the constant-RMR methods $\csownerdsm.\mwait$, $\csownerdsm.\mrelease$, $\csownerdsm.\mread$, $\csownerdsm.\mwrite$, and $\csownerdsm.\mcapture$ in the DSM algorithm, presented in Figure~\ref{algo:dsmfullcrash}.

\item
We have also introduced and implemented a {\em boolean signal object} and replaced each shared variable $\stopwait[i]$ (for $i \in [0,2]$) with a boolean signal object $\stopwaitdsm[i]$, and replaced the earlier algorithm's steps of ``\waittill $\stopwait[i] \isequal \true$'' (at Line 6), ``$\stopwait[i] \leftarrow \true$'' (at Line 25), and ``$\stopwait[i] \gets \mbox{\it false}$ (at Line 23) with the constant-RMR methods $\stopwaitdsm[i].\mwait$, $\stopwaitdsm[i].\mset$, and
$\stopwaitdsm[i].\mreset$.
Compare Lines 6, 23, and 25 of Figures~\ref{algo:fullcrash} and \ref{algo:dsmfullcrash}.

\vspace{0.00in}
\mbox{\hspace{0.3in}}The ``\waittill $\stopwait[\myseqp\%3] \isequal \true$'' appears at both Line 4 and Line 6, but there is a significant difference between the two.
At Line 6, there can be at most one process busy waiting---namely, the winner of $\mlock[\myseqp\%3]$.
In contrast, many processes can be busy waiting at Line 4.
The boolean signal object that we implement supports a single waiting process, hence we use it to handle Line 6, and devise a different mechanism to handle Line 4.

\item
At Line 4 of the CC algorithm, $p$ repeatedly reads the $\stopwait[S_p \% 3]$ variable while performing in parallel the Try method on $\mlock[S_p \% 3]$.
This repeated reading is done because, if a process $q$ installs $\mlock[(S_p+1) \% 3]$ while $p$ is executing the Try method of $\mlock[S_p \% 3]$, the algorithm needs $p$ to detect this development and migrate to the newly installed lock.
To support this detection without incurring unbounded RMRs, we devise a strategy: 
{\sl enter the new, but exit the old}.
In a nutshell, the strategy is to strengthen the starvation-freedom property required of $\mlock[S_p \% 3]$ so that no process ever gets stuck in the lock, so long as all processes---including those that crash while using the $\mlock[S_p \% 3]$---eventually execute the exit section of that lock.
This strategy eliminates the need for the ``wait until'' statement at Line 4 (compare Line 4 of Figure~\ref{algo:fullcrash} with Line 4 of Figure~\ref{algo:dsmfullcrash}), but adds three lines (Lines 9.1, 18.1, and 25.1) where a process executes the exit method on an old lock as it installs or migrates to a new lock.
We explain this strategy in detail soon.


%At Line 4 of the CC algorithm, $p$ repeatedly reads the $\stopwait[S_p \% 3]$ variable while performing in parallel the Try method on $\mlock[S_p \% 3]$.
%This repeated reading is done because, if a process $q$ installs $\mlock[(S_p+1) \% 3]$ while $p$ is executing the Try method of $\mlock[S_p \% 3]$, the algorithm needs to release $p$ from the try section of the old lock, so that $p$ can migrate to the newly installed lock.
%To facilitate this release, we exploit a nice property of our base locks (Figure~\ref{algo:dsmqlock}), as we describe below.

%\mbox{\hspace{0.3in}}
%We recall that the base lock is a queue lock, so processes in the try section of $\mlock[i]$ form a queue.
%Our idea is to ensure that whenever an enqueued process $p$ becomes aware that the next base lock $\mlock[i+1]$ is installed, it releases the process $q$ enqueued immediately behind it by calling $\mlock[i].\exitprocp$, thus setting off a chain reaction that leads to the release of all processes queued behind $p$.
%Since each process $p$ that crashes while active in $\mlock[i]$ will eventually restart and ensure the installation of $\mlock[i+1]$, these chain reactions are bound to start.

%These chains of releases are bound to start because every process $p$ that crashed while active in $\mlock[i]$ will eventually restart and ensure the installation of $\mlock[i+1]$.

%So released, the process $q$ in turn executes $\mlock[i].\texttt{exit}_q()$ to release the process behind it before migrating.
%Thus, the entire chain of processes behind $p$ get released from $\mlock[i]$. 

%When a process $p$ is stuck in the try section of a base lock $\mlock[i]$, it will be released if the process enq 

%{\sl enter the new, but exit the old}.
%In a nutshell, the strategy is to strengthen the starvation-freedom property required of $\mlock[S_p \% 3]$ so that no process ever gets stuck in the lock, so long as all processes---including those that crash while using the $\mlock[S_p \% 3]$---eventually execute the exit section of that lock.
%This strategy eliminates the need for the ``wait until'' statement at Line 4 (compare Line 4 of Figure~\ref{algo:fullcrash} versus Line 4 of Figure~\ref{algo:dsmfullcrash}), but adds three lines (Lines 9.1, 18.1, and 25.1) where a process executes the exit method on an old lock as it installs or migrates to a new lock.
%We explain this strategy in detail soon.
\end{enumerate}

The above ideas give rise to the DSM algorithm in Figure~\ref{algo:dsmfullcrash}, which has three additional lines where $\exitprocp$ is called, as just explained, but every other line corresponds to the same numbered line of the earlier CC algorithm.
The implementations of the capturable object and boolean signal object are in Figures~\ref{algo:capturable} and \ref{algo:dsmsignal} respectively; we describe these later.

\subsection{Handling Line 4}

We now present a scenario that motivates a stronger starvation-freedom property that $\mlock[0..2]$ should support to facilitate the design of our DSM algorithm.

Consider a time $t$ when processes $p$ and $p'$ are in the Try method of $\mlock[i]$, where $S_p = S_{p'} = \seq$ and $i = \seq \% 3$.
Suppose that $p$ is behind $p'$ and is the last process in the ``wait-queue'' of $\mlock[i]$.
Suppose that the system crashes and comes back on subsequently.
Suppose that a process $q$, which had all along been in the remainder section, executes the algorithm.
This process $q$ reads $\seq$ into $S_q$ at Line 3 and executes the Try method of $\mlock[i]$ at Line 4, which causes it to line up behind $p$, which had been previously the last process in the wait-queue of that lock.
Suppose that $p$ now restarts.
It executes the recover method, where it installs the next lock, $\mlock[i+1]$, by incrementing $\seq$ (at Line 24). From then on, any new process $r$ that executes the algorithm will use $\mlock[i+1]$ instead of $\mlock[i]$.
But what about process $q$ which is waiting in $\mlock[i]$'s wait-queue behind $p$?
In the CC algorithm, since $q$ repeatedly checks $\stopwait[i]$, which $p$ sets to {\em true} (at Line 25) after installing the new lock, $q$ will quit Line 4 and migrate to the newly installed $\mlock[i+1]$. Since $q$ cannot afford this repeated check in a DSM machine, we use the following idea instead.
Once $p$ installs a new lock at Line 24 and informs the world that the new lock has been installed (Line 25), we require it to {\em exit} the old lock, $\mlock[i]$, at Line 25.1.
Normally, only a process leaving the critical section of the lock executes the exit section, but in the present case we require all those processes that had crashed while using the lock to also exit the lock so that innocent processes such as $q$ which entered that lock without the knowledge that the lock is not operative would not get stuck.
In particular, in our scenario, $p$'s execution of $\mlock[i]$'s exit wakes up the process $q$ that is waiting behind $p$ in $\mlock[i]$'s wait-queue.
Once awakened, $q$ reads $\seq$ and finds that it is no longer the same as $S_q$ (Line 5), thereby learning that a new lock has been installed, and migrates to the new lock (from Line 5 to Line 9).
As it migrates, $q$ too exits $\mlock[i]$ (at Line 9.1) so that any other process that queued up behind it at $\mlock[i]$ would similarly be able to migrate to the new lock.
In a similar vein, if an exiting process notices
that the next base lock is installed,
it must exit the base lock that it used (at Line 18.1).

Thus, for the DSM algorithm to work, we require that $\mlock[i]$ (for $i \in [0,2])$ supports an $\exitprocp$ method that crashed processes can execute and, when they all do, innocent processes such as $q$ in our scenario do not get stuck in the $\try$ method.  
We capture this requirement by strengthening the starvation-freedom property required of $\mlock[i]$, as follows.

Recall from Section~\ref{mutexspec} that the state of a lock $\ell$ is given by four sets---$\ell.\tryset$, $\ell.\csset$, $\ell.\exitset$, and $\ell.\crashedset$.
To define the stronger starvation-freedom property, we remodel the transition on crash to:

\begin{itemize}
    \item \underline{Transition on System Crash}: When a system crash occurs, all active processes are moved to $\csset$ and added to $\crashedset$, i.e., $\csset$ becomes the union of $\tryset$, $\csset$, and $\exitset$; and $\crashedset$ becomes the union of the four sets---$\tryset$, $\csset$, $\exitset$, and $\crashedset$.
\end{itemize}

In the above, by moving all active processes to $\csset$, we are requiring that all crashed processes, when they subsequently restart, execute the exit section. And by adding all processes to $\crashedset$, the lock ``remembers'' whether any processes crashed in the lock (this is important because, if processes crash in the lock, the lock is exempted from satisfying the Mutual Exclusion requirement).
We strengthen the definition of Starvation-Freedom from the one in Section~\ref{mutexspec} to: 

\begin{itemize}
    \item \underline{Starvation Freedom Despite Crashes}: Every process in $\ell.\tryset$ eventually leaves $\ell.\tryset$, provided that the following standard assumption holds:
    
    \begin{itemize}
        \item[]
        \emph{Assumption $A$}: 
        \begin{itemize}
            \item If $p \in \ell.\csset$, $p$ eventually invokes and executes $\ell.\exit_p()$.
            \item If $p \in \ell.\tryset$ (respectively, $\ell.\exitset$), $p$ eventually executes a step of $\ell.\try_p()$ (respectively, $\ell.\exit_p()$). 
        \end{itemize}
    \end{itemize}

\end{itemize}

\noindent
Lee's algorithm in Figure~\ref{algo:dsmqlock} is a resettable lock that satisfies this stronger starvation-freedom property.
%The result is summarized as:

%\begin{theorem}\label{resetsflock}{\em
%The algorithm in Figure~\ref{algo:dsmqlock} is a resettable %lock that satisfies {\em Starvation Freedom Despite Crashes}.
%It has $O(1)$ RMR complexity on both CC and DSM machines.
%}\end{theorem}

\subsection{Capturable Object: Specification and Implementation}

A {\em capturable object} $\C$ is specified as follows:
$\C.\mbox{\em state}$ is a pid or $\bot$, and
$\C$ supports the following operations.

\begin{itemize}
    \item $\C.\mread$: returns $\C.\mbox{\em state}$.
    \item $\C.\mwrite$: changes $\C.\mbox{\em state}$ to $p$.
    \item $\C.\mrelease$: changes $\C.\mbox{\em state}$ to $\bot$.
    \item $\C.\mcapture$: If $\C.\mbox{\em state} = \bot$, it changes $\C.\mbox{\em state}$ to $p$ and returns {\em true}; otherwise, it returns {\em false}, and leaves $\C.\mbox{\em state}$ unchanged.
    \item $\C.\mwait$: this method returns only if $\C.\mbox{\em state} = \bot$ at some point during the execution of the method. Thus, it is identical to the statement ``wait till $\C.\mbox{\em state} = \bot$''
\end{itemize}

In the algorithm in Figure~\ref{algo:dsmfullcrash}, there are three lines where a process waits on $\csowner$ (Lines 6, 11, 13). In all of these three lines together, for any $i \in \{0, 1, 2\}$, at most one process $p$ executes $\csowner.\mwait{i}$ at any given time.
So, for our purpose, it suffices to implement a capturable object that supports one waiting process at each $i$ (and an arbitrary number of processes that might execute the other operations).
The simple algorithm in Figure~\ref{algo:capturable} efficiently implements such an object, as summarized below:

\input{capturable}

\begin{theorem}{\em
For the algorithm in Figure~\ref{algo:capturable}, if for each $i \in \{0, 1, 2\}$, no two processes execute $\C.\texttt{wait}(i)$ concurrently, then:

\begin{enumerate}
    \item[] 
\begin{itemize}
\item 
$\C$ is linearizable.
\item
The operations $\mread$, $\mwrite$, $\mrelease$, and $\mcapture$ are wait-free.
\item
There is a constant $b$ such that if $\C.\mbox{\em state} = \bot$ at some point in time $t$ and it remains unchanged at $\bot$ from then on, after time $t$ any process $p$ completes any execution of $\C.\mwait$ in at most $b$ of its steps.
\item
A process incurs $O(1)$ RMRs to invoke and complete any of the five operations in both DSM and CC machines.
\end{itemize}
%The algorithm in Figure~\ref{algo:capturable} implements a linearizable capturable object.
%The operations $\mread$, $\mwrite$, $\mrelease$, and $\mcapture$ are wait-free.
%There is a constant $b$ such that if $\C.\mbox{\em state} = \bot$ at some point in time $t$ and it remains unchanged at $\bot$ from then on, after time $t$ any process $p$ completes any execution of $\C.\mwait$ in at most $b$ of its steps.
%Furthermore, $p$ incurs $O(1)$ RMRs to invoke and complete any of the five operations in both DSM and CC machines.
\end{enumerate}

}\end{theorem}

\subsection{Boolean Signal Object: Specification and Implementation}

We have also introduced and implemented a {\em boolean signal object} and replaced each shared boolean $\stopwait[i]$ (for $i \in [0,2]$) with a boolean signal object, and replaced the earlier algorithm's steps of `` \waittill $\stopwait[i] \isequal \true$'' (at Line 6) and ``$\stopwait[i] \leftarrow \true$'' (at Line 25) with the constant-RMR methods $\stopwait[i].\mwait$ and $\stopwait[i].\mset$.

A {\em boolean signal object} $\Sig$ is specified as follows:
$\Sig.\mbox{\em state}$ is Boolean, and
$\Sig$ supports the following three operations.

\begin{itemize}
    \item $\Sig.\mbset$: changes $\Sig.\mbox{\em state}$ to {\em true}.

    \item $\Sig.\mreset$: changes $\Sig.\mbox{\em state}$ to {\em false}

    \item $\Sig.\mbwait$: this method returns only if $\Sig.\mbox{\em state} = \mbox{\em true}$ at some point during the execution of the method. Thus, it is identical to the statement ``wait till $\Sig.\mbox{\em state} = \mbox{\em true}$''
\end{itemize}

In the algorithm in Figure~\ref{algo:dsmfullcrash}, for any $i \in \{0, 1, 2\}$, at most one process $p$ waits on $\stopwait[i]$ (at Line 6) at any given time.
So, for our purpose, it suffices to implement a boolean signal object that supports only one waiting process (and an arbitrary number of setting and resetting processes).
The simple algorithm in Figure~\ref{algo:dsmsignal} efficiently implements such an object, as summarized below:

\input{signal}

\begin{theorem}{\em
For the algorithm in Figure~\ref{algo:dsmsignal}, if for each no two processes execute $\Sig.\texttt{wait}()$ concurrently, then:
\begin{enumerate}
    \item[] 
\begin{itemize}
    \item 
    $\Sig$ is linearizable.
    \item 
    The operations $\mbset$ and $\mreset{}$ are wait-free.
    \item 
    There is a constant $b$ such that if $\Sig.\mbox{\em state} = \mbox{\em true}$ at some point in time $t$ and it remains unchanged at $\mbox{\em true}$ from then on, after time $t$ any process $p$ completes its execution of $\Sig.\mbwait$ in at most $b$ of its steps.
    \item 
    A process incurs $O(1)$ RMRs to invoke and complete any of the three operations in both DSM and CC machines.
\end{itemize}
\end{enumerate}


%If no two processes execute $\Sig.\texttt{wait}()$ concurrently in the algorithm of Figure~\ref{algo:dsmsignal}, then (1) the implementation is linearizable, (2) the operations $\mbset$ and $\mreset{}$ are wait-free, and (3)
%there is a constant $b$ such that if $\Sig.\mbox{\em state} = \mbox{\em true}$ at some point in time $t$ and it remains unchanged at $\mbox{\em true}$ from then on, after time $t$ any process $p$ completes its execution of $\Sig.\mbwait$ in at most $b$ of its steps.
%Furthermore, $p$ incurs $O(1)$ RMRs to invoke and complete any of the three operations in both DSM and CC machines.
}\end{theorem}

\subsection{The final result}

The theorem below summarizes the results of this paper.

\begin{theorem}{\em
	The algorithm in Figure~\ref{algo:dsmfullcrash} solves the recoverable mutual exclusion problem on DSM and CC machines for an arbitrary number of processes of arbitrary names.
	It satisfies mutual exclusion, bounded exit, bounded critical section reentry, and starvation freedom.
	The space complexity of the algorithm is $O(1)$ per process, and
	the RMR complexity of the algorithm on DSM and CC machines is $O(1)$ per passage.
}\end{theorem}

\noindent
{\em Proof}: The algorithm in Figure~\ref{algo:dsmfullcrash} has the same invariant as that in Figure~\ref{algo:fullcrash}, and the proofs of the properties are accordingly the same.
\hfill $\square$



==> introduction-old.tex <==
\section{Introduction}

The emergence and widespread commercial availability of {\em non-volatile memory (NVM)}, which retains its state despite {\em system-wide crashes} caused by power outages \cite{nvmm:pcm, nvmm:memristor, nvmm:mram} has ushered in the era of {\em durable} algorithms, which allow processes that {\em crash}, and lose the contents of their process registers due to a system-wide power outage, to smoothly {\em recover} upon {\em restart} and resume computing from the time of the crash  \cite{IzraelevitzMS16, attiya:rlin, FriedmanHMP18, FriedmanPetrankRamalhete, Golab:rmutex, Golab:rmutex2, Golab:rmutex3, Golab:rmutex, jayanti:fasasmutex, jayanti:rmesublog, jayanti:fcfsmutex, jayanti:rmeabort, Chan, ChanWoelfelLB}.
Due to the centrality of {\em mutual exclusion (mutex)} locks in concurrent computing \cite{Dijkstra:mutex}, the {\em recoverable mutual exclusion (RME) problem} has received a lot of attention  \cite{Golab:rmutex, Golab:rmutex2, Golab:rmutex3, Golab:rmutex, jayanti:fasasmutex, jayanti:rmesublog, jayanti:fcfsmutex, jayanti:rmeabort, Chan, ChanWoelfelLB}.
The principal goal of RME lock research has been to design algorithms that have low ``RMR'' and space complexity for both {\em cache-coherent (CC)} and {\em distributed shared memory (DSM)} systems, even in the face of crashes.
%As first observed by Golab and Ramaraju \cite{Golab:rmutex}, a most fundamental synchronization tool in concurrent computing that benefits from a {\em recoverable} counterpart is the {\em mutual exclusion (mutex) lock} \cite{Dijkstra:mutex}.
In this paper, we design an efficient RME lock that overcomes system-wide crashes, allows threads of arbitrary names, and has just constant worst-case RMR complexity for both CC and DSM systems, while requiring just constant space per process.

\paragraph{\bf Failure models}
Recoverable algorithms for {\em system-wide failure}, have been widely studied in both the theory and systems communities \cite{IzraelevitzMS16, Golab:rmutex3, FriedmanHMP18, FriedmanPetrankRamalhete, LiGolab, ConditNightingaleFrostIpek, CoburnEtAlConference, CoburnEtAlJournal, KolliPelleySaidiChenWenisch}.
System-wide failures are caused by power-outages and cause all processes in the system to crash simultaneously.
A lot of theory literature, particularly related to RME, has also studied the {\em individual crash model} \cite{Golab:rmutex2, Golab:rmutex, jayanti:fasasmutex, jayanti:rmesublog, jayanti:fcfsmutex, jayanti:rmeabort, Chan, ChanWoelfelLB, BenDavid, Attiya}, in which individual processes can crash and restart even as other processes run unaffected.
Algorithms designed for the individual crash model work in the system-wide crash model, because a system-wide crash can be simulated as a sequence of individual crashes.
Algorithms designed directly for the system-wide crash model however, can exploit the structure in the simultaneous failure to potentially achieve better efficiency guarantees.
The main result of this paper---a constant worst-case RMR algorithm for RME in the system-wide crash model---displays such an efficiency boost in light of Chan and Woelfel's $\Omega(\log n / \log\log n)$ worst-case RMR lower bound for RME in the individual crash model.

\subsection{Recoverable Mutual Exclusion: Problem Statement}

A standard mutex lock $\ell$ consists of two methods ---$\ell.\mbox{\em try}_p()$ and 
$\ell.\mbox{\em exit}_p()$ for each process $p$---and
a {\em recoverable} mutex lock consists of one additional method, called $\ell.\mbox{\em recover}_p()$.
Initially each process is in the {\em remainder section} and in a {\em correct} state.
From the remainder section, when in the correct state a process $p$ may invoke and execute $\ell.\mbox{\em try}_p()$.
When $\ell.\mbox{\em try}_p()$ returns, $p$ is said to be in the {\em critical section (CS)}.
From the CS, $p$ must next invoke and execute $\ell.\mbox{\em exit}_p()$.
When this method completes, $p$ is back in the remainder section and in the correct state.

At any time, a process can execute a {\em normal step} or a system-wide crash can occur.
In a normal step of a process $p$, $p$ executes the instruction pointed to by its program counter $\pcp$.
When a crash occurs, for each process $p$,  $\pcp$ is set to $p$'s remainder section and 
all other $p$'s registers and all $p$'s local variables that are not in the NVM are set to arbitrary values.
% The system might crash at any point in time.
If the process $p$ is outside the Remainder section at the time of crash, the crash event puts $p$ in Remainder section and in the ``crashed'' state.
When $p$ subsequently restarts, it is required to invoke and execute $\ell.\mbox{\em recover}_p()$.
When this method completes, it returns either $\gotorem$ or $\gotocs$ and puts $p$ back in the correct state.
A return value of $\gotorem$ by $\ell.\mbox{\em recover}_p()$ puts $p$ in the remainder section and a return value of $\gotocs$ puts $p$ in the CS.
If $p$ crashed in the CS, the subsequent execution of recover that returns, must put $p$ back in the CS.
A process is said to be {\em active} from the time it leaves the remainder section in the correct state to the earliest subsequent time when it returns to the remainder section in the correct state.
A {\em run} of an algorithm is an infinite sequence of steps and crashes.

%We assume that the CS is bounded and idempotent.

\paragraph{\bf Properties}
Our RME algorithm satisfies the following properties:

\begin{itemize}
	\item
	\underline{Mutual Exclusion}: At most one process is in the CS at any time.
	\item
	\underline{Bounded Exit}: There is a constant $c$ such that,
	if any process $p$ executes the steps of $\ell.\mbox{\em exit}_p()$
	without any intervening crash steps,
	$p$ returns from $\ell.\mbox{\em exit}_p()$ in at most $c$ of its steps.
	
	\item
	\underline{Bounded Critical Section Reentry}: There is a constant $c$ such that,
	if a crash occurs while a process $p$ is in the CS, then $p$ reenters the CS 
	before it executes $c$ of its steps that have no intervening crash steps.
	
	\item
	\underline{Starvation Freedom}: In every infinite fair run, if a process $p$ invokes 
	$\ell.\mbox{\em try}_p()$ at any time $t$, it is in the Remainder in the correct state at some time $t' > t$,
	where we call an infinite run {\em fair} if,
	only a finite number of crash events occur in the run, 
	no process stays in the CS forever, and when not in the Remainder in the correct state,
	no process permanently stops taking steps.

	%\underline{Starvation Freedom}: In every fair run, if a process $p$ invokes 
	%$\ell.\mbox{\em try}_p()$ at any time $t$, it is in the Remainder at some time $t' > t$,
	%where we call a run {\em fair} if it is infinite,
	%only a finite number of crash events occur in the run, 
	%no process stays in the CS forever, and %when not in the Remainder,
	%no process permanently stops taking steps.
\end{itemize}

\paragraph{\bf Multiprocessor Models and Passage and Super-passage Complexity}
The complexity of mutual exclusion algorithms is commonly studied in two multiprocessor models:
{\em cache-coherent} (CC) and {\em distributed shared memory} (DSM).

In the CC model, each process has a cache.
A read operation by a process $p$ on a shared variable $X$ fetches a copy of $X$ from 
shared memory to $p$'s cache, if a copy is not already present in the cache.
Any non-read operation on $X$ by any process invalidates copies of $X$ at all caches.
An operation on $X$ by $p$ counts as a
{\em remote memory reference} (RMR) if either the operation is not a read
or $X$'s copy is not already present in $p$'s cache.
When a process crashes, its cache contents are lost.

In the DSM model, shared memory is partitioned between the processes.
Each shared variable $X$ resides in exactly one of the parts.
{\em Any} operation on $X$ by a process $p$ counts as an RMR if and only if $X$ is not in $p$'s part of shared memory.

A {\em passage} of a process $p$ in a run starts from the time it leaves the remainder (in the correct or the crashed state) to the earliest subsequent time when $p$ returns to the remainder
(in the correct or the crashed state).

A {\em super-passage} of a process $p$ in a run starts when $p$ either leaves the remainder for the first time
in the run or when $p$ leaves the remainder for the first time after its previous super-passage has ended,
and it ends when $p$ subsequently returns to the remainder by completing $\ell.\mbox{\em exit}_p()$.

The {\em passage complexity} (respectively, {\em super-passage complexity})
of an RME algorithm is the worst-case number of RMRs that a process incurs
in a passage (resp., super-passage). 
We use the term RMR complexity interchangeably with passage complexity.

\paragraph{\bf Dynamic Joining and Adaptive Space Complexity}
Previous RME locks have been designed for a fixed set of $N$ processes labeled $1,\ldots,N$, and have required pre-allocated shared-arrays of length $N$ for communication.
We introduce, to our knowledge, the first RME lock to allow {\em dynamic joining}, i.e., newly created processes of arbitrary names (a.k.a. threads) can be created on-the-fly, and these processes can access our locks.
To achieve this property, we design all communication structures in our protocol to be pointer-based, so we can eliminate the need for pre-allocated fixed-length arrays.
We ensure that our space usage only grows in the actual number of processes $n$ that use our lock.

%The {\em RMR complexity} of a mutex lock $\ell$ is
%the worst case number of RMRs that a process incurs between the time 
%it invokes $\ell.\mbox{\em recover}_p()$ to the earliest subsequent time that it returns to the remainder section
%(either because of a crash event or because it completes $\ell.\mbox{\em exit}_p()$).


%\subsection{What makes designing recoverable algorithms hard?}

%Constant worst-case RMR locks for the standard (i.e., non-recoverable) mutex problem have been long known.
%The famous MCS-lock \cite{MCS:mutex}, and its several variants \cite{}, all have this property.
%At first glance, it might seem that recoverable algorithms are simple to design if we simply let processes store all of their information in NVM.
%For instance, consider the strategy where all local and shared variables are stored in NVM and every process stores its program counter's value in NVM after each instruction.
%Does this strategy make recovery from crashes easy?
%In particular, when processes restart after a crash, can they simply consult the stored state to learn where to resume their execution from?
%The answer is no.
%To see why, suppose that the crash occurs immediately after a process $p$ performs the instruction $r \leftarrow \mbox{\em FAS}(X, v)$ (if $X$'s value is $u$ immediately before the instruction, this instruction writes $u$ in the CPU register $r$ and updates $X$'s value to $v$).
%Since we said the crash occurs immediately after $p$ performs this instruction (and before $p$ records in NVM the value $u$ of register $r$), the wiping out of the CPU registers by the crash event causes irretrievable loss of the value written in the register $r$.
%So, when $p$ subsequently restarts, it cannot fully restore its state, nor would it be correct for $p$ to repeat the FAS instruction.
%In fact, overcoming this problem can be challenging and costly.
%For instance, while it is well known that $O(1)$ worst-case RMR complexity is achievable for non-recoverable mutex \cite{MCS:mutex, craig:mcs, dvir:mutex, jayanti:jjjqlock, lee:twonodeme},  RME in the {\em individual crash model} requires at least $\Omega(\log n/\log\log n)$ RMRs in the worst-case \cite{ChanWoelfelLB}.

\subsection{Our contributions}
We design two RME algorithms for the system-wide crash model.
Our first algorithm has $O(1)$ worst-case RMR complexity in the CC model and requires $O(1)$ space per process.
Our second algorithm has $O(1)$ worst-case RMR complexity in both the CC and DSM models and also requires just $O(1)$ space per process.
Both algorithms allow for dynamic joining, and only require the standard {\em fetch-and-store (FAS)} and {\em compare-and-swap (CAS)} instructions for synchronization.\footnote{The operation $r \leftarrow \mbox{\bf FAS}(X, v)$ has the following semantics: if $X$'s value is $u$ immediately before the instruction, it writes $u$ in the CPU register $r$ and updates $X$'s value to $v$. The operation $r \gets \mbox{\bf CAS}(X, u, v)$ has the following semantics: 
if $X$'s value is $u$, the operation changes $X$'s value to $v$ and writes {\em true} in the CPU register $r$;
otherwise, $X$ remains unchanged and the operation writes {\em false} in $r$.}

\subsection{Comparison to the state of the art}
Four previous works explore the possibility of constant RMR solutions for RME locks.
Two of the works require hardware support for an instruction that atomically manipulates two un-related words of shared-memory called {\em FASAS fetch-and-store-and-store}  to achieve $O(1)$ worst-case RMR complexity RME algorithms in the individual process crash model \cite{Golab:rmutex2, jayanti:fasasmutex}.
To our knowledge, no current systems support this instruction.
Chan and Woelfel designed an RME algorithm for the independent crash model, which achieves {\em amortized} $O(1)$ RMR complexity and requires unbounded space \cite{Chan}.
The lower bound by the same author \cite{ChanWoelfelLB} shows that $O(1)$ {\em worst-case} RMR complexity cannot be achieved in the individual crash model, and confirms that the worst-case $\Theta(\log n/\log\log n)$ RMR algorithms of Golab and Hendler \cite{Golab:rmutex2} and Jayanti et al. \cite{jayanti:rmesublog} are the best possible for CC and DSM in that model of computation.
Golab and Hendler (GH) designed a pair of RME algorithms for the system-wide crash model, which assume that ``processes receive additional information from the environment regarding the occurrence of the failure,'' to achieve $O(1)$ worst-case RMR \cite{Golab:rmutex3}.
Specifically, the GH algorithms assume that processes have access to a shared failure-counter, which an out-of-band environmental mechanism must increase after each crash event.
Their CC algorithm can be implemented with constant space per process, and the DSM algorithm requires $O(N)$ space per process, i.e., $O(N^2)$ space over $n$ processes.
The GH algorithms also achieves  {\em failures robust fairness}, which states that in an infinite run with infinitely many successful super passages, every process that executes the try section eventually reaches the critical section.
%The GH algorithms also achieve a new fairness property define by them called  {\em failures robust fairness}, which states that in an infinite run with infinitely many successful super passages, every process that executes the try section eventually reaches the critical section, even if there are infinitely many system-wide crashes.

To our knowledge, our algorithms are the only RME locks to achieve worst-case $O(1)$ RMR complexity assuming nothing more than standard hardware support. 
They are also the first to achieve dynamic joining.
Furthermore, in light of Chan and Woelfel's $\Omega(\log n / \log\log n)$ worst-case RMR lower bound for RME in the individual crash model, our results show a separation between the system-wide crash and individual crash models in worst-case RMR complexity in both the CC and DSM models (without assuming a failure detector).

\subsection{Related research on RME}
Golab and Ramaraju formalized the RME problem and designed several algorithms by adapting traditional mutual exclusion algorithms \cite{Golab:rmutex}.
Ramaraju \cite{ramaraju:rglock}, Jayanti and Joshi \cite{jayanti:fcfsmutex}, and Jayanti et al. \cite{jayanti:fasasmutex} 
designed RME algorithms that support the First-Come-First-Served property \cite{Lamport:fcfsmutex}.
Golab and Hendler \cite{Golab:rmutex2} and Jayanti et al. \cite{jayanti:rmesublog} presented RME algorithms that have sub-logarithmic RMR complexity.
Recently, Jayanti and Joshi \cite{jayanti:rmeabort} designed an RME algorithm that has the abort capability.
Dhoked and Mittal gave a lock with sub-logarithmic RMR complexity that is additionally adaptive \cite{Mittal}.
A recent lower bound by Chan and Woelfel \cite{ChanWoelfelLB} matches the upper bounds of Jayanti et al. \cite{jayanti:rmesublog} and Golab and Hendler \cite{Golab:rmutex2} to pin down the worst-case RMR complexity of RME in the individual crash model as $\Theta(\log n/\log\log n)$ for both the CC and DSM models.
Interestingly, Chan and Woelfel's previous work shows that, given unbounded space, $O(1)$ RMR complexity can be achieved in the {\em amortized} sense. 
All these results apply to the individual crash model of failure.
As discussed above, Golab and Hendler \cite{Golab:rmutex3} presented an algorithm that has $O(1)$ RMR complexity in the system-wide crash model of failure, assuming a failure detector.

\subsection{Paper Overview}
In the remainder of the paper, we first introduce a standard, non-recoverable base lock that we use as a subroutine in our algorithm.
Then, we describe an RME algorithm that has all the desired properties but only for CC machines.
Finally, we describe how to transform this algorithm into one that is efficient in both the CC and DSM models.
We end with some concluding remarks.
%TODO: Add the following citations that Wojciech pointed out:
% (1)    Ryan Berryhill, Wojciech M. Golab, Mahesh Tripunitara: Robust Shared Objects for Non-Volatile Main Memory. OPODIS 2015: 20:1-20:17
% (2)    Joseph Izraelevitz, Hammurabi Mendes, Michael L. Scott: Linearizability of Persistent Memory Objects Under a Full-System-Crash Failure Model. DISC 2016: 313-327
% The first paper discusses wait-freedom and recoverability, and overlaps directly with Attiya et al.
% Attiya et al. \cite{attiya:rlin} and Ben-David et al. \cite{naama:casobj} present linearizable implementations of recoverable objects.



==> mutex_spec_old.tex <==
\section{Two Resettable (Non-Recoverable) Mutual Exclusion Locks}\label{mutexspec}

In Figures~\ref{algo:qlock} and \ref{algo:dsmqlock} we present the well known standard (non-recoverable) queue locks due to Lee \cite{lee:twonodeme} with just one line added to support a reset method.
We call these two locks {\em resettable} locks, and employ these in the design of our recoverable mutual exclusion algorithms for CC and DSM described in the next sections.


%The two main algorithms of this paper (described in the next sections) use `` resettable'' standard mutex locks.
%Informally, a (non-recoverable) resettable lock behaves like a standard mutex lock, but makes no guarantee of any properties if processes crash while using the lock. However, the lock supports a method to reset it to the initial state. 
%We present a more careful definition below.


%To design the main algorithms of this paper, we use standard (non-recoverable) locks that 

%A main result of this paper, which we present in the next section, is an algorithm that transforms any non-recoverable, but {\em resettable} mutex lock $L$ into a {\em recoverable} mutex lock that, in the CC model, has the same RMR complexity as $L$. Informally, a (non-recoverable) resettable lock behaves like a standard mutex lock, but makes no guarantee of any properties if processes crash while using the lock. However, the lock supports a method to reset it to the initial state. 
%We present a more careful definition below.
 
Each resettable lock $\ell$ supports $\ell.\try()$, $\ell.\exit()$, and an atomic (i.e. single-line) $\ell.\reset()$ method.
We describe the status of processes using four sets: $\ell.\tryset$, $\ell.\csset$, $\ell.\exitset$, and $\ell.\crashedset$.
Initially, all four sets are empty.
%We let $\activeset$ denote the union of $\tryset$, $\csset$, and $\exitset$.
The changes in the sets due to the invocation or return from $\ell.\try()$ or $\ell.\exit()$, a crash event, and the execution of $\ell.\reset()$ are as follows:

\begin{itemize}
    \item 
    A process $p$ may invoke $\try_p()$ only if $p \not\in \tryset \cup \csset \cup \exitset \cup \crashedset$; this invocation adds $p$ to $\tryset$.
    Furthermore, $p$ may perform a step of $\try_p()$ only if $p \in \tryset$.
    Finally, if $p$ returns from $\try_p()$, then $p$ is removed from $\tryset$ and added to $\csset$.
    
    \item 
    A process $p$ may invoke $\exit_p()$ only if $p \in \csset$; this invocation removes $p$ from $\csset$ and adds $p$ to $\exitset$.
    Furthermore, $p$ may perform a step of $\exit_p()$ only if $p \in \exitset$.
    Finally, if $p$ returns from $\exit_p()$, then $p$ is removed from $\exitset$.

    \item 
    When a system crash occurs, all active processes are moved to $\crashedset$, i.e., $\crashedset$ becomes the union of the four sets---$\tryset \cup \csset \cup \exitset \cup \crashedset$---and the other three sets become empty.

    \item 
    A process $p$ may execute $\reset_p()$ only if $\tryset \cup \csset \cup \exitset = \varnothing$;
    this execution causes all four sets to become empty, i.e. $\tryset = \csset = \exitset = \crashedset = \varnothing$.
    
    %When $p \not \in \ell.\tryset \cup \ell.\csset \cup \ell.\exitset$, $p$ may invoke $\ell.\try_p()$. Upon invoking $\ell.\try_p()$, $p$ is added to $\ell.\tryset$ and $p$ may start executing the steps of $\ell.\try_p()$.
    %\item When $p \in \ell.\tryset$ and the method $\ell.\try_p()$ returns, $p$ moves from $\ell.\tryset$ to $\ell.\csset$.
    %\item When $p \in \ell.\csset$ and invokes $\ell.\exit_p()$, $p$ moves from $\ell.\csset$ to $\ell.\exitset$ and $p$ may start executing the steps of $\ell.\exit_p()$.
    %\item When $p \in \ell.\exitset$ and the method $\ell.\exit_p()$ returns, $p$ is removed from $\ell.\exitset$.
    %\item When a system crash occurs, all active processes are moved to $\ell.\crashedset$, i.e., $\ell.\crashedset$ becomes the union of the four sets---$\ell.\tryset$, $\ell.\csset$, $\ell.\exitset$, and $\ell.\crashedset$---and the other three sets become empty.
    %\item When $\ell.\tryset \cup \ell.\csset \cup \ell.\exitset$ is empty, any process $p$ may execute $\ell.\reset_p()$.
    %When a process $p$ executes $\ell.\reset_p()$, all of $\ell.\tryset$, $\ell.\csset$, $\ell.\exitset$, and $\ell.\crashedset$ become/remain empty.
    %\item When $\ell.\tryset \cup \ell.\csset \cup \ell.\exitset$ is empty, any process $p$ is free to call $\ell.\exit_p()$.
    %When process $p$ executes $\ell.\exit_p()$ the sets remain unchanged.
\end{itemize}

The properties, RMR complexities, and space complexities of the resettable locks are summarized in the following two theorems.

\begin{theorem}{\em 
A {\em resettable lock} $\ell$, i.e. an algorithm from Figure~\ref{algo:qlock} or \ref{algo:dsmqlock}, satisfies the following properties:

\begin{itemize}
    \item \underline{Mutual Exclusion}: If $\ell.\crashedset$ is empty, then $\ell.\csset$ contains at most one process.
    
    \item \underline{Starvation Freedom}: If a process $p$ is in $\ell.\tryset$ at time $t$ and $\ell.\crashedset$ is empty at all times $t' \ge t$, then $p$ eventually leaves $\ell.\tryset$, provided that the following standard assumption holds:
    
    \begin{itemize}
        \item[]
    \emph{Assumption $A$}: 
    \begin{itemize}
        \item If $p \in \ell.\csset$, $p$ eventually invokes $\ell.\exit_p()$.
        \item If $p \in \ell.\tryset$ (respectively, $\ell.\exitset$), $p$ eventually executes a step of $\ell.\try_p()$ (respectively, $\ell.\exit_p()$). 
    \end{itemize}
    \end{itemize}

    
    \item \underline{Bounded Exit and Bounded Reset}: Each process $p$ completes $\ell.\exit_p()$ and $\ell.\reset_p()$ in a bounded number of its steps.
    
    \item \underline{Correct Reset}: If a process $p$ executes $\ell.\reset_p()$, then $\ell$ returns to an initial state.
    
    %Informally, the reset method resets a lock to its initial state.
    %Our results in this paper are valid even with a weak guarantee that reset works correctly only under the condition that no process executes a Try or Exit step while a Reset method is in progress. Specifically:
    
    %\begin{itemize}
    %\item[] 
    % Once a process $p$ invokes $\ell.\reset_p()$, the reset method is considered to be in progress until either $p$ returns from the method or the system crashes. If no process $q$ performs a step of $\ell.\try_q()$ while $\ell.\reset_p()$ is in progress, when $\ell.\reset_p()$ returns, $\ell$ is in the initial state. (Note that multiple processes may execute the reset method concurrently.)
    %\end{itemize}

\end{itemize}
}\end{theorem}

%It is trivial to convert a traditional lock into a resettable one by adding a reset method that simply writes the initial values in shared variables.
%This idea works since all we need is a {\em weak} reset.
%In Figures~\ref{algo:qlock} and \ref{algo:dsmqlock} we present the well known queue locks due to Lee \cite{lee:twonodeme} with just one line added to support the reset method.
%We summarize the result thus:

\begin{theorem}\label{resetlock}
{\em 
The resettable lock algorithm in Figures~\ref{algo:qlock} has $O(1)$ RMR complexity in CC machines, the resettable lock algorithm in Figure~\ref{algo:dsmqlock} has $O(1)$ RMR complexity in both CC and DSM machines, and both resettable locks have $O(1)$ space complexity per process.
}
\end{theorem}

\input{resettable}
\input{abandonable}


% Since queue-locks are well known, we do not describe here how they work, but Appendix ??? contains a description. 



==> specification.tex <==
\section{Specification of the problem} \label{ch2:spec}

In the traditional Mutual Exclusion (ME) problem \cite{Dijkstra:mutex}, there are asynchronous processes
that repeatedly compete for exclusive access to a shared resource. 
For example, a process $p$ does this by repeatedly cycling through four sections of code:
Remainder, Try (as a procedure $\tryprocp()$), Critical, and Exit (as a procedure $\exitprocp()$) sections. 
When in Remainder, $p$ may need access to the shared resource which can be obtained only after getting exclusive ownership of the Critical Section (henceforth referred as CS). 
Thus, $p$ invokes $\tryprocp()$, which, upon returning, makes $p$ the owner of the CS so that $p$ can access the shared resource.
Once $p$ has finished accessing the shared resource, $p$ has to relinquish its ownership of the CS so that the CS remains available subsequently. 
To this purpose, $p$ invokes $\exitprocp()$ where it gives up its ownership of the CS and goes back to the Remainder upon returning. 
Hence, an algorithm for the ME problem gives code for $\tryprocp()$ and $\exitprocp()$ for every process $p$, so that
processes can gain exclusive access to the CS (while satisfying certain fairness conditions).
An assumption here is that $p$ will not crash while executing $\tryprocp()$, $\exitprocp()$, or CS.

Our system consists of asynchronous processes that communicate by applying
operations on shared memory locations (with NVM being the shared memory). 
The failure model of the system, referred to as the {\em crash-restart model}, is as follows. 
A process can crash from time to time. 
When a process $p$ crashes, all of $p$’s registers lose their contents, 
i.e., $p$’s program counter is reset to a default location $\ell$ in $p$’s program, 
and all other registers of $p$ are changed to arbitrary values. 
However, any shared variable stored in the NVM is unaffected by a crash and retains its values. 
A crashed process $p$ eventually restarts, executing the program beginning from the instruction at the default location $\ell$, 
regardless of where in the program $p$ might have crashed prior to the restart.

Suitably adapting the ME problem to the crash-restart model gives rise to a new problem as follows, for which we present algorithms in this thesis.
In the {\em Recoverable Mutual Exclusion (RME) problem}, each process may repeatedly crash at any point (including in CS or anywhere else in the code for the algorithm solving the problem) 
and restart at some later point.
When a process $p$ crashes, $p$'s program counter is reset to the Remainder Section and 
the values of $p$'s remaining registers are lost; 
however, the values of the variables stored in the NVM remain in tact.
When $p$ subsequently restarts, it executes a recovery method, called the Recover ($\recoverprocp()$) section.
The purpose of $\recoverprocp()$ is to fix any broken parts of the algorithm that $p$’s crash may have caused and allow $p$ to go back
to cycle through the remaining four sections of code as discussed above for ME. 
Hence, an algorithm designed for the RME problem gives code for $\tryprocp()$, $\exitprocp()$, and $\recoverprocp()$ for every process $p$.

The {\em Abortable RME} problem enhances the RME problem 
by requiring an additional feature whereby a process waiting for the CS,
when signaled by the environment, can abandon its wait and quickly return to the Remainder.

In this section, we rigorously specify the Abortable RME problem by defining
(1) what an abortable RME algorithm is,
(2) modeling the algorithm's executions, and
(3) the properties that these executions must satisfy.
Towards the end of the section we discuss how a specification for the RME and ME problems can be obtained from this specification of the Abortable RME problem.

\subsection{Abortable RME algorithm}


\begin{definition}[Abortable RME algorithm] \label{ch2:armespec}
	{\em 
		An {\em Abortable Recoverable Mutual Exclusion algorithm}, abbreviated {\em Abortable RME algorithm}, 
		is a tuple $(\procset, \varset, \valset, \initmap, \operations, \partition, \methods)$, where
		
		\begin{itemize}
			\item
			$\procset$ is a set of processes.
			Each process $p \in \procset$ has a set of registers,
			including a {\em program counter}, denoted $\pcp$,
			which points to an instruction in $p$'s code.
			
			\item
			$\varset$ is a set of variables,
			which includes a Boolean variable $\abortsigp$, for each $p \in \mathcal{P}$.
			No process except $p$ can invoke any operation on $\abortsigp$,
			and $p$ can only invoke a read operation on $\abortsigp$.
			
			Intuitively, the ``environment''  sets  $\abortsigp$ to $\true$
			when it wishes to communicate to $p$ that it should abort its attempt to acquire the CS and return to the Remainder.
			
			\item
			$\valset$ is a set of values (that each variable in $\varset$ can possibly take on).
			For example, on a 64-bit machine, $\valset$ would be the set of all 64-bit integers. 
			
			\item
			$\initmap$ is a function that assigns a value from $\valset$ to each variable in $\varset$.
			For all $X \in \varset$, we say $\initmap(X)$ is $X$'s {\em initial value}.
			
			\item
			$\operations$ is a set of operations that each variable in $\varset - \{\abortsigp \mid p \in \procset \}$ supports.
			
			Our algorithms assume that $\operations$ includes {\em read}, {\em write}, and
			one or both of {\em compare\&swap} (\cas) and {\em fetch\&store} (\fas),
			described as follows.
			In the following, $X$ denotes a variable in $\varset$, and 
			$r$ and $s$ denote the registers of a process that executes the operation.
			
			\begin{itemize}
				\item
				read$(X)$, which returns the value of $X$.
				
				\item
				write$(X,r)$, which writes in $X$ the value of $r$.
				
				\item
				\fas$(X, r)$, which writes in $X$ the value of $r$ and returns $X$'s previous value.
				
				\item
				\cas$(X, r, s)$, which compares the values of $X$ and $r$; 
				if they are equal, writes in $X$ the value in $s$ and returns $\true$;
				otherwise, returns $\false$, leaving $X$ unchanged.
			\end{itemize}
			
			\item
			$\partition$ is a partition of $\varset$ into $|\procset|$ sets, named $\partition(p)$, for each $p \in \procset$.
			Intuitively, $\partition(p)$ is the set of variables that reside locally at process $p$ in a DSM architecture.
			
			\item
			$\methods$ is a set of methods, which includes 
			three methods per process $p \in \procset$, named $\tryprocp()$, $\exitprocp()$, and $\recoverprocp()$, such that:
			\begin{itemize}
				\item
				In any instruction of any method, 
				at most one operation is performed and 
				it is performed on a single variable from $\varset$.
				\item
				The methods $\tryprocp()$ and $\recoverprocp()$ return a value from $\{\gotocs, \gotorem\}$, and
				$\exitprocp()$ has no return value.
				
				\item
				None of $\tryprocp()$, $\exitprocp()$, or $\recoverprocp()$ calls itself or the other two.
				(This assumption simplifies the model, but is not limiting in any way because 
				it does not preclude the use of helper methods that can call themselves or the others.)
			\end{itemize}
		\end{itemize}
	}
\end{definition}

For each process $p \in \procset$, we model $p$'s code outside of the methods in $\methods$
to consist of two disjoint sections, named $\remprocp()$ and $\critsecp()$.  

Informally, when $\tryprocp()$ or $\recoverprocp()$ returns $\gotorem$ or when $\exitprocp()$ completes,
$\pcp$ is set to $\remprocp()$;
and when $\tryprocp()$ or $\recoverprocp()$ returns $\gotocs$, $\pcp$ is set to $\critsecp()$.
The $\tryprocp()$ method may return $\gotorem$ only in response to an abort signal to $p$ from the ``environment''.

Process $p$ executes $\recoverprocp()$ when it restarts after a crash.
The purpose of the recover method is to ``repair'' the adverse effects of the crash
and put $p$ back where it belongs.
For example, if $p$ crashes while in the CS,
the subsequent execution of $\recoverprocp()$ launches $p$ back into the CS by returning $\gotocs$.
On the other hand, if $p$ crashes while executing $\tryprocp()$,
$\recoverprocp()$ has a choice---it can either roll $p$ back to the Remainder
by returning $\gotorem$ or put it in the CS by returning $\gotocs$.
Similarly, if $p$ crashes while executing $\exitprocp()$,
$\recoverprocp()$ has a choice of returning either $\gotorem$ or $\gotocs$.


\subsection{Modeling an algorithm's execution} \label{ch2:executionmodel}

Let $\algotuple = (\procset, \varset, \valset, \initmap, \operations, \partition, \methods)$ be an abortable RME algorithm.
We formalize in this section the notion of a {\em run}, which captures what can transpire when
$\algotuple$ is executed on a machine. 
For each process $p \in \procset$:

\begin{itemize}
	\item
	We model $p$'s code outside of the methods in $\methods$
	to consist of two disjoint sections, named $\remprocp()$ and $\critsecp()$.
	
	\item
	We model $p$'s ``recovery status'' with $\status_p$
	that can take on any one of five values---$\good$, $\rectry$, $\reccs$, $\recexit$, or $\recrem$.
	($\status_p$ is an ``abstract variable'' in the sense that it is not in $\varset$
	and hence is not accessed by the methods in $\methods$;
	its purpose is merely to help define the problem.)
	
	Informally, if $\status_p \neq \good$, it means that $p$ is still recovering from a crash,
	and in this case, the value of $\status_p$ reveals where the crash occured.
	
	\item
	We introduce an ``abstract'' variable $\cache_p$, 
	which holds a set of pairs of the form $(X, v)$,
	where $X \in \varset$ and $v \in \valset$.
	We call $\cache_p$ an abstract variable because it is not in $\varset$ and, hence,
	not manipulated directly by the code.
	It is introduced to help define what operations count as {\em remote memory references} (RMR)  on
	CC machines.
\end{itemize}

The rules governing when $p$ can invoke the $\tryprocp()$, $\exitprocp()$, and $\recoverprocp()$ methods,
and how $\status_p$ and $\pcp$ are affected by crash and other events will be formally captured
soon in the definition of a run, but first we state these rules informally as follows:

\begin{itemize}
	
	\item
	If $p$ is in the Remainder and $\status_p = \good$, 
	$p$ either invokes $\tryprocp()$ and enters the Try section or invokes $\recoverprocp()$ and enters the Recover section.
	
	When $\tryprocp()$ completes, it returns either $\gotocs$ or $\gotorem$.
	If $\tryprocp()$ returns $\gotocs$, $p$ enters the CS, i.e., $\pcp$ is set to $\critsecp()$.
	On the other hand, if $\tryprocp()$ returns $\gotorem$, $p$ enters the Remainder, i.e., $\pcp$ is set to $\remprocp()$.
	
	\item
	If $p$ is in the CS, it invokes $\exitprocp()$ and enters the Exit section.
	When $\exitprocp()$ returns, $p$ enters the Remainder, i.e., $\pcp$ is set to $\remprocp()$.
	
	\item
	If $p$ crashes while in the Try section (respectively, CS or Exit section),
	$\status_p$ switches from $\good$ to $\rectry$ (respectively, $\reccs$ or $\recexit$),
	$\pcp$ is set to $\remprocp()$, and $p$'s all other registers are set to arbitrary values.
	
	\item
	If $p$ is in the Remainder and $\status_p \neq \good$, $p$ invokes $\recoverprocp()$ and enters the Recover section.
	
	\item
	When $p$ is in the Recover section, both $\status_p = \good$ and $\status_p \neq \good$ are possible
	(the former is possible if $p$ invokes $\recoverprocp()$ when in the Remainder with $\status_p = \good$).
	If $p$ crashes in the Recover section when $\status_p \neq \good$,
	$\status_p$ remains unchanged, 
	$\pcp$ is set to $\remprocp()$, and $p$'s all other registers are set to arbitrary values.
	On the other hand, if $p$ crashes in the Recover section when $\status_p = \good$,
	$\status_p$ switches to $\recrem$, 
	$\pcp$ is set to $\remprocp()$, and $p$'s all other registers are set to arbitrary values.
	
	\item
	When $\recoverprocp()$ completes, it returns either $\gotocs$ or $\gotorem$.
	If $\recoverprocp()$ returns $\gotocs$, $p$ enters the CS and $\status_p$ is set to $\good$.
	On the other hand, if $\recoverprocp()$ returns $\gotorem$, $p$ enters the Remainder
	and $\status_p$ is set to $\good$.
\end{itemize} 
\noindent In what follows, we formalize the above informal notions.

\begin{definition}[State of a process] \label{ch2:def:state}
	{\em
		A {\em state} of a process $p$ is a function that assigns a value
		to each of $p$'s registers, including $\pcp$, and a value to each of $p$'s abstract variables---$\status_p$, $\abortsigp$, and $\cache_p$.
	}
\end{definition}

\begin{definition}[Configuration] \label{ch2:def:config}
	{\em
		A {\em configuration} is a function that assigns a state to each process in $\procset$
		and a value to each variable in $\varset$.
	}
\end{definition}

Intuitively, a configuration is a snapshot of the algorithm's state at a point in time.

\begin{definition}[Initial configuration] \label{ch2:def:initconfig}
	{\em
		An {\em initial configuration} is a configuration, which, for each $p \in \procset$, 
		assigns $\pcp = \remprocp()$, $\status_p = \good$, $\abortsigp = \false$, $\cache_p = \emptyset$,
		and, for each $X \in \varset$, $X = \initmap(X)$.
	}
\end{definition}

\begin{definition}[Run] \label{ch2:def:run}
	{\em
		A {\em run} is a finite sequence 
		$C_0, \alpha_1, C_1, \alpha_2, C_2,  \ldots \alpha_{k}, C_k$, or
		an infinite sequence $C_0, \alpha_1, C_1, \alpha_2, C_2, \ldots$ such that:
		
		\begin{enumerate}
			\item
			$C_0$ is an initial configuration and,
			for each $i$, $C_i$ is a configuration and $\alpha_i$ is either one of $(p, \normal)$ or $(p, \crash)$, for some $p \in \procset$, or just $\crash$.
			
			
			We call each triple $(C_{i-1}, \alpha_i, C_i)$ a {\em step};
			it is a {\em normal step of $p$} if $\alpha_i = (p, \normal)$,
			it is a {\em crash step of $p$} (also called individual crash of $p$) if $\alpha_i = (p, \crash)$,
			and it is a {\em system crash step} if $\alpha_i = \crash$.
			
			\item
			For each normal step $(C_{i-1}, (p, \normal), C_i)$, we have:
			
			\begin{itemize}
				\item
				If $\pcp = \remprocp()$ and $\status_p = \good$, then $C_i$ is the configuration that results
				from $p_i$ invoking either $\tryprocp()$ or $\recoverprocp()$ from configuration $C_{i-1}$.
				If $p$ invokes $\tryprocp()$ (respectively, $\recoverprocp()$),
				we say $p$ enters the Try (respectively, Recover) section in this step.
				In the configuration that follows the step when $p$ enters the Try (respectively, Recover) section, i.e., in $C_i$ in this case,
				$\pcp$ points to the first instruction of $\tryprocp()$ (respectively, $\recoverprocp()$).
				
				\item
				If $\pcp = \remprocp()$ and $\status_p \neq \good$, then $C_i$ is the configuration that results
				from $p_i$ invoking $\recoverprocp())$ from configuration $C_{i-1}$.
				We say $p$ enters the Recover section in this step.
				In the configuration that follows the step when $p$ enters the Recover section, i.e., in $C_i$ in this case,
				$\pcp$ points to the first instruction of $\recoverprocp()$.
				
				\item
				If $\pcp = \critsecp()$, then $C_i$ is the configuration that results
				when $p_i$ invokes $\exitprocp()$ from configuration $C_{i-1}$.
				We say $p$ enters the Exit section in this step.
				In the configuration that follows the step when $p$ enters the Exit section, i.e., in $C_i$ in this case,
				$\pcp$ points to the first instruction of $\exitprocp()$.
				
				\item
				Otherwise, $C_i$ is the configuration that results
				when $p_i$ executes the instruction that $\pcp$ points to in configuration $C_{i-1}$.
				If this instruction returns $\gotocs$ (respectively, $\gotorem$), then 
				$\pcp$ is set to $\critsecp()$ (respectively, $\remprocp()$) in $C_i$, and
				we say $p$ enters the CS (respectively, Remainder) in this step.
				Furthermore, if in this instruction $p$ returns from $\recoverprocp()$,
				$\status_p$ is set to $\good$ in $C_i$.
			\end{itemize}
			
			\item
			For each individual crash step $(C_{i-1}, (p, \crash), C_i)$, we have:
			
			\begin{itemize}
				\item
				In $C_i$, $\pcp$ is set to $\remprocp()$, $\cache_p$ is set to $\emptyset$, and all other registers of $p$ are set to arbitrary values.
				
				\item
				If $\status_p \neq \good$ in $C_{i-1}$, then $\status_p$ remains unchanged in $C_i$.
				Otherwise, if $p$ is in the Try section (respectively, CS, Exit, or Recover section),
				then $\status_p$ is set to $\rectry$ (respectively, $\reccs$, $\recexit$, or $\recrem$) in $C_i$.
			\end{itemize}
			
			\item
			For each system crash step $(C_{i-1}, \crash, C_i)$, we have, for each $p \in \procset$:
			
			\begin{itemize}
				\item
				In $C_i$, $\pcp$ is set to $\remprocp()$, $\cache_p$ is set to $\emptyset$, and all other registers of $p$ are set to arbitrary values.
				
				\item
				If $\status_p \neq \good$ in $C_{i-1}$, then $\status_p$ remains unchanged in $C_i$.
				Otherwise, if $p$ is in the Try section (respectively, CS, Exit, or Recover section),
				then $\status_p$ is set to $\rectry$ (respectively, $\reccs$, $\recexit$, or $\recrem$) in $C_i$.
			\end{itemize}
			
			\item
			A step $(C_{i-1}, \alpha_i, C_i)$ is an RMR in a DSM machine if and only if 
			$\alpha_i$ performs an operation on some $X \in \varset$ in that step and for the process $p \in \procset$ executing the operation from step $\alpha_i$, $X \not \in \partition(p)$.
			
			\item
			A step $(C_{i-1}, \alpha_i, C_i)$ is an RMR in the CC machine if and only if 
			$\alpha_i$ performs a non-read operation or
			$\alpha_i$ reads some $X \in \varset$ and 
			for the process $p \in \procset$ executing the operation from step $\alpha_i$, $\cache_p$ does not contain a pair of the form $(X, *)$.
			Furthermore, if $\alpha_i$ reads $X$ in the step, the pair $(X,v)$ is inserted in $\cache_p$,
			where $v$ is $X$'s value in $C_{i-1}$.
			Finally, if $\alpha_i$ performs a non-read operation on $X$ in the step,
			then any pair of the form $(X, *)$ is removed from $\cache_q$, for all $q \in \procset$.
			
		\end{enumerate}
	}
\end{definition}

Note, in the definition above we discussed two types of crash steps: individual crash and system crash.
Algorithms presented in Chapter~\ref{ch3} and \ref{ch4} assume that crashes are only individual process crashes, and
the algorithm presented in Chapter~\ref{ch5} assumes that a crash is a system crash only.

\begin{definition}[Fair run] \label{ch2:def:fairrun}
	{\em
		A run $R = C_0, \alpha_1, C_1, \alpha_2, C_2,  \ldots$ is {\em fair} if and only if either $R$ is finite or, 
		for all configurations $C_i$ and for all processes $p \in \procset$, the following condition is satisfied:
		if $\pcp \neq \remprocp()$ in $C_i$,
		then $p$ has a step in the suffix of $R$ from $C_i$.
	}
\end{definition}

This definition captures that in a fair run, no process ceases to take steps when it is outside the Remainder section.
This implies that no process stays in the CS forever and no process halts permanently in the Try or Exit sections.

\begin{definition}[Passage] \label{ch2:def:passage}
	{\em
		A {\em passage} of a process $p$ is a contiguous sequence $\sigma$ of steps in a run such that
		$p$ leaves $\remprocp()$ (i.e., $\pcp$ changes from $\remprocp()$) in the first step of $\sigma$ and the last step of $\sigma$ is the earliest
		subsequent step in the run where $p$ reenters $\remprocp()$ (i.e., $\pcp$ changes to $\remprocp()$).
	}
\end{definition}

\begin{definition}[Attempt] \label{ch2:def:attempt}
	{\em
		An {\em attempt} of a process $p$ is a maximal contiguous sequence $\sigma$ of steps in a run such that
		$p$ leaves $\remprocp()$ in the first step of $\sigma$ with $\status_p = \good$ and the last step of $\sigma$ is the earliest
		subsequent step in the run where $p$ reenters $\remprocp()$ due to a normal step with $\status_p = \good$ 
		(or $\status_p$ gets set to $\good$ as a consequence of the step, e.g., due to return from $\recoverprocp()$ to $\remprocp()$).
	}
\end{definition}

\begin{definition}[Passage RMR complexity]
	{\em
		The {\em CC Passage RMR complexity} (respectively, {\em DSM Passage RMR complexity})
		is the maximum number of steps that count as RMRs in the CC model (respectively, DSM model)
		in a single passage of any process in any run.
	}
\end{definition}

\begin{definition}[Attempt RMR complexity]
	{\em
		The {\em CC Attempt RMR complexity} (respectively, {\em DSM Attempt RMR complexity})
		is the maximum number of steps that count as RMRs in the CC model (respectively, DSM model)
		in a single attempt of any process in any run.
	}
\end{definition}

The RMR complexity of an algorithm is a function of $n$, the number of processes in the system (i.e., $|\procset|$), and $f$, the number of crashes a process incurs during an attempt.

\subsection{Desirable properties} \label{ch2:properties}

We now state the desirable properties of an abortable RME algorithm,
which we divide into three groups---general, recovery-related, and abort-related.

\begin{definition}[General properties] \label{ch2:def:basicprop}
	{\em
		\mbox{ }
		
		\begin{itemize}
			\item[P1]
			\underline{Mutual Exclusion}: At most one process is in the CS in any configuration of any run.
			
			\item[P2]
			\underline{Bounded Exit}: There is an integer $b$ such that if in any run any process $p$ invokes
			and executes $\exitprocp()$ without crashing, the method completes in at most $b$ steps of $p$.
			
			\item[]
			We present two versions of starvation-freedom.
			%\begin{itemize}
			\item[P3]
			\underline{Weak Starvation Freedom (WSF)}: In every fair infinite run in which there are only finitely many crash steps,
			if a process $p$ is in the Try section in a configuration, $p$ is in a different section in a later configuration.
			\item[P4]
			\underline{Starvation Freedom (SF)}: In every fair infinite run in which every attempt contains 
			only finitely many crash steps,
			if a process $p$ is in the Try section in a configuration, $p$ is in a different section in a later configuration.
			%\end{itemize}
			
			We note that SF implies WSF.
			
			\item[P5]
			\underline{First-Come-First-Served (FCFS)}:
			There is an integer $b$ such that in any run,
			if $A$ and $A'$ are attempts by any distinct processes $p$ and $p'$, respectively,
			$p$ performs at least $b$ consecutive normal steps in $A$ before the attempt $A'$ starts, 
			and $p$ does neither receive an abort signal nor subsequently crash in $\tryprocp()$ in $A$,
			then $p'$ does not enter the CS in $A'$ before $p$ enters the CS in $A$.
			
			We note that an algorithm might not always satisfy FCFS property. 
			In fact the results from Chapter~\ref{ch4} and \ref{ch5} do not always satisfy this property.
		\end{itemize}
	}
\end{definition} 

\begin{definition}[Recovery properties] \label{ch2:def:recprop}
	{\em
		\mbox{ }
		
		\begin{itemize}
			\item[P6]
			\underline{Critical Section Reentry (CSR) \cite{Golab:rmutex}}:
			In any run, if a process $p$ crashes while in the CS, 
			no other process enters the CS until $p$ subsequently reenters the CS.
			
			\item[P7]
			\underline{Bounded Recovery to CS/Exit}:
			There is an integer $b$ such that if in any run any process $p$ 
			executes $\recoverprocp()$ without crashing and with $\status_p \in \{\reccs, \recexit\}$, 
			the method completes in at most $b$ steps of $p$.
			
			\item[P8]
			\underline{Fast Recovery to Remainder}:
			There is a constant $b$ (independent of $|\procset|$) such that if in any run any process $p$ 
			executes $\recoverprocp()$ without crashing and with $\status_p \in \{\good, \recrem\}$, 
			the method completes in at most $b$ steps of $p$.
			
			\item[P9]
			\underline{Bounded Recovery to Remainder}:
			There is an integer $b$ such that if in any run
			$\recoverprocp()$, executed by a process $p$ with $\status_p = \rectry$, returns $\gotorem$,
			$p$ must have completed that execution of $\recoverprocp()$ in at most $b$ of its steps.
		\end{itemize}
	}
\end{definition}


We next define the correctness properties related to the abort capability supported by the algorithm.
First we define a predicate $\beta$ as follows:
for any run $R$, any configuration $C$ of $R$, and any process $p$,
$\beta(R, p, C)$ is $\true$ if and only if in configuration $C$
it is the case that $\abortsigp$ is $\true$ and
either $p$ is in the Try section or $p$ is in the Recover section with $\status_p = \rectry$.

\begin{definition}[Abort properties] \label{ch2:def:abortprop}
	{\em
		\mbox{ }
		
		\begin{itemize}
			\item[P10]
			\underline{Bounded Abort}: 
			There is an integer $b$ such that, for each $R, C, p$,
			if $\beta(R, p, C)$ is true,
			$\abortsigp$ stays $\true$ for ever (i.e., stays true in the suffix $R'$ of the run from $C$), 
			and $p$ executes steps without crashing (i.e., $p$ has no crash steps in $R'$),
			then $p$ enters either the CS or the remainder in at most $b$ of its steps (in $R'$).
			
			\item[P11]
			\underline{No Trivial Aborts}: 
			In any run, if $\abortsigp$ is $\false$ when a process $p$ invokes $\tryprocp()$,
			$\abortsigp$ remains $\false$ forever, and $p$ executes steps without crashing,
			then $\tryprocp()$ does not return $\gotorem$.
		\end{itemize}
	}
\end{definition}


\subsection{Why is the design of recoverable algorithms nontrivial?}

At first glance, it might seem that recoverable algorithms are simple to design
if we let processes store all of their information in NVM.
For instance, consider the strategy where all local and shared variables are stored in NVM and
every process stores its program counter's value in NVM after each instruction.
It would be interesting to know whether this strategy makes recovery from crashes easy?
When processes restart after a crash, can they simply consult the stored state to learn where to resume their execution from?
The answer is no.
To see why, suppose that the crash occurs immediately after
a process $p$ performs the instruction $r \leftarrow \mbox{\em FAS}(X, v)$
(if $X$'s value is $u$ immediately before the instruction,
this instruction writes $u$ in the CPU register $r$ and updates $X$'s value to $v$).
Since we said the crash occurs immediately after $p$ performs this instruction (and
before $p$ records in NVM the value $u$ of register $r$), 
the wiping out of the CPU registers by the crash event causes irretrievable loss of the value written in the register $r$.
This loss can be catastrophic, as is the case in the MCS algorithm, where the loss of the return value from \mbox{\em FAS} on the {\em Tail} of 
the queue of waiting processes disconnects that queue, leading to live-lock.
So, when processes subsequently restart, they can't restore the state.
Thus, even when NVM is available, the design of recoverable algorithms is nontrivial.

\subsection{Our contribution and comparison to the state of the art}

We design a recoverable mutual exclusion algorithm for the CC multiprocessors
that meets the same gold standard of performance under system-wide crashes
as that set by MCS for failure-free systems.
In particular, our algorithm supports an arbitrary number of processes of arbitrary names,
it has $O(1)$ RMR-complexity, and
it can be used to implement $m$ locks, shared by $n$ processes,
using only $O(m+n)$ words of memory if each process releases the lock 
it previously acquired before attempting to acquire a new lock.
Our algorithm also satisfies bounded critical section reentry, as well as
bounded exit and starvation-freedom properties.
Our algorithm uses the FAS and CAS operations, the same operations used in MCS.
(We explained FAS earlier. The operation CAS$(X, u, v)$ has the following semantics: 
if $X$'s value is $u$, the operation changes $X$'s value to $v$ and returns {\em true} to $p$;
otherwise, $X$ remains unchanged and the operation returns {\em false} to $p$.)

Golab and Hendler's paper \cite{Golab:rmutex3} is the only other work that we are aware of 
that uses realistic shared memory operations and
still achieves $O(1)$ RMR complexity for recoverable mutual exclusion.
The comparison to their algorithm is as follows:

\begin{itemize}
	\item
	Golab and Hendler's algorithm (GH) too works only for only the system-wide crash model,
	but theirs works for both the CC and DSM models (in contrast, ours works only for CC).
	\item
	GH does not support an arbitrary number of processes:
	when GH is deployed, it must be instantiated with any specific number $n$,
	and then it can only support at most $n$ processes.
	\item
	Using GH to implement $m$ locks, shared by $n$ processes, requires $O(mn^2)$ space.
	In contrast, if each process accesses a lock only after relinquishing a previously acquired lock,
	our algorithm needs only $O(m+n)$ space (and without the ``at most one lock at a time for each process''
	requirement, our algorithm needs $O(mn)$ space).
\end{itemize}

Aside from the above, the two works differ on one significant aspect:
GH makes the assumption that processes have access to a counter and 
the environment somehow ensures that the value of this counter increases after each crash event.
Our algorithm does not rely on any such assumption.

\subsection{Related research}
Golab and Ramaraju \cite{Golab:rmutex} formalized the RME problem and designed several algorithms by adapting traditional mutual exclusion algorithms.
Ramaraju \cite{ramaraju:rglock}, Jayanti and Joshi \cite{jayanti:fcfsmutex}, and Jayanti et al. \cite{jayanti:fasasmutex} 
designed RME algorithms that support the First-Come-First-Served property \cite{Lamport:fcfsmutex}.
Golab and Hendler \cite{Golab:rmutex2} and Jayanti et al. \cite{jayanti:rmesublog} presented RME algorithms that has sub-logarithmic RMR complexity.
Recently, Jayanti and Joshi \cite{jayanti:rmeabort} designed an RME algorithm that has the abort capability.
All these results apply to the individual crash model of failure.
As discussed above, Golab and Hendler \cite{Golab:rmutex3} presented an algorithm that has $O(1)$ RMR complexity in the system-wide crash model of failure.

%TODO: Add the following citations that Wojciech pointed out:
% (1)    Ryan Berryhill, Wojciech M. Golab, Mahesh Tripunitara: Robust Shared Objects for Non-Volatile Main Memory. OPODIS 2015: 20:1-20:17
% (2)    Joseph Izraelevitz, Hammurabi Mendes, Michael L. Scott: Linearizability of Persistent Memory Objects Under a Full-System-Crash Failure Model. DISC 2016: 313-327
% The first paper discusses wait-freedom and recoverability, and overlaps directly with Attiya et al.
Attiya et al. \cite{attiya:rlin} and Ben-David et al. \cite{naama:casobj} present linearizable implementations of recoverable objects.

